Wave packet treatment of neutrino flavour and spin oscillations in galactic and extragalactic magnetic fields

We consider neutrino flavour and spin oscillations in a magnetic field using formalism of wave packets. Decoherence effects due to neutrino wave packets separation are studied. The considered effects are especially important for describing astrophysical neutrino oscillations, since they propagate on kiloparsec scale and bigger. The obtained results are of interest for neutrino telescopes IceCube, Baikal-GVD and KM3NeT, and also can be applied for description of supernovae neutrino oscillations effects would be detected by JUNO and Hyper-Kamiokande.

==> Popov_Studenikin_ACHEP <==
SyncTeX Version:1
Input:1:D:\Science\2024_ACHEP\samplepaper.tex
Input:2:D:\Science\2024_ACHEP\llncs.cls
Input:3:C:\Users\artem\AppData\Local\Programs\MiKTeX 2.9\tex\latex\base\article.cls
Input:4:C:\Users\artem\AppData\Local\Programs\MiKTeX 2.9\tex\latex\base\size10.clo
Input:5:C:\Users\artem\AppData\Local\Programs\MiKTeX 2.9\tex\latex\tools\multicol.sty
Input:6:C:\Users\artem\AppData\Local\Programs\MiKTeX 2.9\tex\latex\oberdiek\aliascnt.sty
Input:7:C:\Users\artem\AppData\Local\Programs\MiKTeX 2.9\tex\latex\base\fontenc.sty
Input:8:C:\Users\artem\AppData\Local\Programs\MiKTeX 2.9\tex\latex\graphics\graphicx.sty
Input:9:C:\Users\artem\AppData\Local\Programs\MiKTeX 2.9\tex\latex\graphics\keyval.sty
Input:10:C:\Users\artem\AppData\Local\Programs\MiKTeX 2.9\tex\latex\graphics\graphics.sty
Input:11:C:\Users\artem\AppData\Local\Programs\MiKTeX 2.9\tex\latex\graphics\trig.sty
Input:12:C:\Users\artem\AppData\Local\Programs\MiKTeX 2.9\tex\latex\graphics-cfg\graphics.cfg
Input:13:C:\Users\artem\AppData\Local\Programs\MiKTeX 2.9\tex\latex\graphics-def\pdftex.def
Input:14:C:\Users\artem\AppData\Local\Programs\MiKTeX 2.9\tex\latex\tools\bm.sty
Input:15:C:\Users\artem\AppData\Local\Programs\MiKTeX 2.9\tex\latex\l3backend\l3backend-pdftex.def
Input:16:D:\Science\2024_ACHEP\samplepaper.aux
Input:17:C:\Users\artem\AppData\Local\Programs\MiKTeX 2.9\tex\context\base\mkii\supp-pdf.mkii
Input:18:C:\Users\artem\AppData\Local\Programs\MiKTeX 2.9\tex\latex\epstopdf-pkg\epstopdf-base.sty
Input:19:C:\Users\artem\AppData\Local\Programs\MiKTeX 2.9\tex\latex\00miktex\epstopdf-sys.cfg
Input:20:C:\Users\artem\AppData\Local\Programs\MiKTeX 2.9\tex\latex\base\t1cmtt.fd
Output:pdf
Magnification:1000
Unit:1
X Offset:0
Y Offset:0
Content:
!1733
{1
[1,61:4736286,45574276:26877856,40837990,0
(1,61:4736286,4736286:0,0,0
[1,61:0,4736286:0,0,0
(1,61:0,0:0,0,0
g1,61:0,0
)
]
)
[1,61:8865054,45574276:22749088,39789414,0
[1,61:8865054,6571294:22749088,786432,0
(1,61:8865054,6571294:22749088,0,0
h1,61:8865054,6571294:22749088,0,0
)
]
[1,61:8865054,43608196:22749088,35988326,0
(1,40:8865054,8275230:22749088,651269,183455
k1,40:9531746,8275230:666692
(1,40:9531746,8275230:0,0,0
g1,40:9531746,8275230
g1,40:9531746,8275230
g1,40:9204066,8275230
h1,40:9204066,8275230:0,0,0
g1,40:9531746,8275230
)
x1,40:10603515,8275230
x1,40:11035948,8275230
x1,40:11554869,8275230
x1,40:11997933,8275230
g1,40:12343881,8275230
x1,40:13900646,8275230
x1,40:14419567,8275230
x1,40:15266236,8275230
g1,40:15612184,8275230
x1,40:19744773,8275230
x1,40:20119549,8275230
g1,40:20465497,8275230
x1,40:21301537,8275230
g1,40:21647485,8275230
x1,40:25481156,8275230
g1,40:25827104,8275230
x1,40:26922605,8275230
x1,40:27441526,8275230
x1,40:28929421,8275230
g1,40:29275369,8275230
x1,40:30947450,8275230
k1,40:31614142,8275230:666692
)
(1,40:8865054,9454878:22749088,651269,183455
k1,40:10054617,9454878:1189563
x1,40:11905438,9454878
g1,40:12251386,9454878
x1,40:17221498,9454878
g1,40:17567446,9454878
x1,40:18432315,9454878
g1,40:18778263,9454878
x1,40:22237737,9454878
g1,40:22583685,9454878
x1,40:24255766,9454878
g1,40:24601714,9454878
x1,40:30424580,9454878
k1,40:31614142,9454878:1189562
)
(1,40:8865054,10634526:22749088,651269,183455
k1,40:16853096,10634526:7988042
x1,40:20957438,10634526
g1,40:21303386,10634526
x1,40:23626100,10634526
g1,40:23626100,10634526
k1,40:31614142,10634526:7988042
)
(1,40:8865054,12912707:22749088,533465,127400
k1,40:14169825,12912707:5304771
x1,40:16009845,12912707
g1,40:16228245,12912707
x1,40:16674145,12912707
x1,40:17347545,12912707
x1,40:17693345,12912707
x1,40:18020945,12912707
$1,40:18020945,12912707
(1,40:18020945,12674882:294003,295640,0
x1,40:18282180,12674882
)
$1,40:18314948,12912707
g1,40:18533348,12912707
x1,40:19588948,12912707
g1,40:19807348,12912707
x1,40:22721168,12912707
g1,40:22939568,12912707
x1,40:26015368,12912707
$1,40:26015368,12912707
(1,40:26015368,12674882:294003,295640,0
x1,40:26276603,12674882
)
$1,40:26309371,12912707
g1,40:26309371,12912707
k1,40:31614142,12912707:5304771
)
(1,40:8865054,14286252:22749088,406224,114660
k1,40:15537497,14286252:6672443
h1,40:15537497,14286252:0,0,0
x1,40:18493813,14286252
x1,40:18712666,14286252
g1,40:18914686,14286252
x1,40:19402901,14286252
g1,40:19604921,14286252
x1,40:22603368,14286252
g1,40:22805388,14286252
x1,40:23554500,14286252
x1,40:24941700,14286252
g1,40:24941700,14286252
k1,40:31614142,14286252:6672442
)
(1,40:8865054,15007148:22749088,406224,114660
k1,40:13677415,15007148:4812361
h1,40:13677415,15007148:0,0,0
x1,40:15347354,15007148
x1,40:15768227,15007148
g1,40:15970247,15007148
x1,40:17350943,15007148
g1,40:17552963,15007148
x1,40:18832331,15007148
x1,40:19965232,15007148
x1,40:20268261,15007148
x1,40:20386105,15007148
g1,40:20588125,15007148
x1,40:22406305,15007148
g1,40:22608325,15007148
x1,40:24278264,15007148
x1,40:24867487,15007148
g1,40:25069507,15007148
x1,40:26801781,15007148
g1,40:26801781,15007148
k1,40:31614142,15007148:4812361
)
(1,40:8865054,15728044:22749088,360360,131040
k1,40:12654839,15728044:3789785
h1,40:12654839,15728044:0,0,0
x1,40:20084807,15728044
g1,40:20394389,15728044
x1,40:27824357,15728044
g1,40:27824357,15728044
k1,40:31614142,15728044:3789785
)
(1,44:10729733,17702016:19019730,407043,114660
(1,42:10729733,17702016:3190817,407043,0
g1,42:10729733,17702016
g1,42:10729733,17702016
g1,42:10402053,17702016
(1,42:10402053,17702016:3190817,407043,0
g1,42:10402053,17702016
g1,42:10729733,17702016
x1,42:13592870,17702016
)
g1,42:13920550,17702016
)
x1,42:14476014,17702016
k1,43:14702475,17702016:226461
x1,43:15682270,17702016
k1,43:15908731,17702016:226461
x1,43:16548461,17702016
x1,43:16885161,17702016
x1,43:17408638,17702016
k1,43:17635099,17702016:226461
x1,43:18072808,17702016
x1,43:18325560,17702016
k1,43:18552021,17702016:226461
x1,43:19461110,17702016
x1,43:20711858,17702016
k1,43:20938320,17702016:226462
x1,43:21881308,17702016
x1,43:23162131,17702016
k1,43:23388592,17702016:226461
x1,43:24028322,17702016
x1,43:24331351,17702016
x1,43:25191299,17702016
k1,43:25417760,17702016:226461
x1,43:26394190,17702016
k1,43:26620651,17702016:226461
x1,43:27701457,17702016
k1,43:27927918,17702016:226461
x1,43:28470004,17702016
x1,43:29076063,17702016
x1,43:29547443,17702016
x1,43:29749463,17702016
k1,44:29749463,17702016:0
)
(1,44:10729733,18422912:19019730,406224,114660
x1,44:12012558,18422912
k1,43:12238495,18422912:225937
x1,43:12743545,18422912
k1,43:12969481,18422912:225936
x1,43:13272511,18422912
k1,43:13498448,18422912:225937
x1,43:14609558,18422912
x1,43:15889244,18422912
k1,43:16115180,18422912:225936
x1,43:17226518,18422912
k1,43:17452455,18422912:225937
x1,43:18028211,18422912
x1,43:18836291,18422912
k1,43:19062227,18422912:225936
x1,43:19787496,18422912
x1,43:20763926,18422912
x1,43:21676382,18422912
k1,43:21902319,18422912:225937
x1,43:22390534,18422912
k1,43:22616470,18422912:225936
x1,43:23054179,18422912
x1,43:23340373,18422912
x1,43:23643402,18422912
x1,43:23896154,18422912
k1,43:24122091,18422912:225937
x1,43:25031180,18422912
x1,43:25334209,18422912
x1,43:26230056,18422912
k1,43:26455992,18422912:225936
x1,43:27188497,18422912
x1,43:27760886,18422912
x1,43:28604228,18422912
x1,43:29749463,18422912
k1,43:29749463,18422912:0
)
(1,44:10729733,19143808:19019730,406224,114660
x1,44:10999321,19143808
x1,44:12366548,19143808
k1,43:12633544,19143808:266996
x1,43:13576532,19143808
k1,43:13843528,19143808:266996
x1,43:14382247,19143808
k1,43:14649243,19143808:266996
x1,43:15592231,19143808
x1,43:16873054,19143808
k1,43:17140050,19143808:266996
x1,43:17577759,19143808
x1,43:17863953,19143808
x1,43:18166982,19143808
x1,43:18419734,19143808
k1,43:18686730,19143808:266996
x1,43:19595819,19143808
x1,43:19898848,19143808
x1,43:20626345,19143808
k1,43:20893341,19143808:266996
x1,43:21738685,19143808
x1,43:22041715,19143808
x1,43:22581799,19143808
x1,43:23625568,19143808
k1,43:23892564,19143808:266996
x1,43:24702236,19143808
k1,43:24969232,19143808:266996
x1,43:26117377,19143808
x1,43:27060365,19143808
k1,43:27327361,19143808:266996
x1,43:28371358,19143808
k1,43:28638354,19143808:266996
x1,43:29547443,19143808
x1,43:29749463,19143808
k1,44:29749463,19143808:0
)
(1,44:10729733,19864704:19019730,406224,114660
x1,44:11473839,19864704
x1,44:12586769,19864704
k1,43:12780300,19864704:193531
x1,43:13049888,19864704
x1,43:14417115,19864704
k1,43:14610646,19864704:193531
x1,43:15420318,19864704
k1,43:15613849,19864704:193531
x1,43:16122493,19864704
x1,43:16459193,19864704
x1,43:16745616,19864704
x1,43:18142920,19864704
k1,43:18336451,19864704:193531
x1,43:19009851,19864704
x1,43:19346551,19864704
x1,43:19903470,19864704
x1,43:20778889,19864704
x1,43:20997742,19864704
k1,43:21191273,19864704:193531
x1,43:21916542,19864704
k1,43:22110073,19864704:193531
x1,43:22716361,19864704
x1,43:23966880,19864704
x1,43:24774960,19864704
k1,43:24968491,19864704:193531
x1,43:25510577,19864704
x1,43:26286350,19864704
x1,43:26959750,19864704
x1,43:27501835,19864704
x1,43:27670185,19864704
x1,43:28410924,19864704
k1,43:28604455,19864704:193531
x1,43:29547443,19864704
x1,43:29749463,19864704
k1,44:29749463,19864704:0
)
(1,44:10729733,20585600:19019730,406224,114660
x1,44:12010556,20585600
k1,43:12269382,20585600:258826
x1,43:12811468,20585600
x1,43:13417527,20585600
x1,43:13888907,20585600
x1,43:15340082,20585600
k1,43:15598908,20585600:258826
x1,43:16881961,20585600
k1,43:17140787,20585600:258826
x1,43:18302629,20585600
k1,43:18561455,20585600:258826
x1,43:19774939,20585600
x1,43:20077969,20585600
x1,43:21189306,20585600
k1,43:21448132,20585600:258826
x1,43:22087862,20585600
k1,43:22346688,20585600:258826
x1,43:23306283,20585600
x1,43:24183067,20585600
x1,43:24961070,20585600
k1,43:25219896,20585600:258826
x1,43:26469279,20585600
k1,43:26728105,20585600:258826
x1,43:27704535,20585600
k1,43:27963361,20585600:258826
x1,43:28771441,20585600
x1,43:29749463,20585600
k1,43:29749463,20585600:0
)
(1,44:10729733,21306496:19019730,406224,114660
x1,44:11773730,21306496
k1,43:12041565,21306496:267835
x1,43:12950654,21306496
x1,43:13694760,21306496
x1,43:14807690,21306496
k1,43:15075525,21306496:267835
x1,43:15345113,21306496
x1,43:16712340,21306496
k1,43:16980175,21306496:267835
x1,43:17789847,21306496
k1,43:18057682,21306496:267835
x1,43:18545897,21306496
k1,43:18813733,21306496:267836
x1,43:18982083,21306496
x1,43:19318783,21306496
x1,43:20044278,21306496
x1,43:20788611,21306496
k1,43:21056446,21306496:267835
x1,43:21781715,21306496
k1,43:22049550,21306496:267835
x1,43:22992538,21306496
x1,43:24273361,21306496
k1,43:24541196,21306496:267835
x1,43:25484411,21306496
x1,43:26632556,21306496
x1,43:27158035,21306496
k1,43:27425870,21306496:267835
x1,43:28183581,21306496
x1,43:29294690,21306496
x1,43:29749463,21306496
k1,43:29749463,21306496:0
)
(1,44:10729733,22027392:19019730,406224,0
x1,44:11950225,22027392
x1,43:12589954,22027392
x1,43:13982890,22027392
g1,43:14184910,22027392
x1,43:15161340,22027392
g1,43:15363360,22027392
x1,43:18023242,22027392
k1,44:29749463,22027392:11726221
g1,44:29749463,22027392
)
(1,46:10729733,23404612:19019730,407043,114660
x1,46:12468060,23404612
x1,45:13942130,23404612
x1,45:16825780,23404612
g1,45:17027800,23404612
x1,45:17196150,23404612
g1,45:17398170,23404612
x1,45:19739734,23404612
g1,45:19941754,23404612
x1,45:22844104,23404612
g1,45:23046124,23404612
x1,45:23214474,23404612
g1,45:23416494,23404612
x1,45:25559176,23404612
x1,45:26946376,23404612
k1,46:29749463,23404612:2803087
g1,46:29749463,23404612
)
(1,50:8865054,25307265:22749088,542724,0
(1,50:8865054,25307265:1326780,509964,0
g1,50:8865054,25307265
x1,50:9307314,25307265
g1,50:10191834,25307265
)
x1,50:11012654,25307265
x1,50:12135593,25307265
x1,50:15059423,25307265
k1,50:31614142,25307265:16554719
g1,50:31614142,25307265
)
(1,52:8865054,26621841:22749088,451360,127400
x1,52:9356454,26621841
k1,51:9531679,26621841:175225
x1,51:9972119,26621841
k1,51:10147345,26621841:175226
x1,51:11184745,26621841
x1,51:12003745,26621841
k1,51:12178970,26621841:175225
x1,51:13380170,26621841
k1,51:13555395,26621841:175225
x1,51:14687435,26621841
x1,51:15473675,26621841
x1,51:15746675,26621841
k1,51:15921901,26621841:175226
x1,51:16941101,26621841
x1,51:17634521,26621841
x1,51:18584561,26621841
k1,51:18759786,26621841:175225
x1,51:19123786,26621841
x1,51:19728026,26621841
x1,51:20794546,26621841
k1,51:20969771,26621841:175225
x1,51:21661371,26621841
x1,51:22025371,26621841
x1,51:23046391,26621841
x1,51:23737991,26621841
k1,51:23913217,26621841:175226
x1,51:24968817,26621841
x1,51:25807837,26621841
x1,51:27009037,26621841
x1,51:28392237,26621841
k1,51:28567462,26621841:175225
x1,51:29515682,26621841
x1,51:29879682,26621841
x1,51:30445702,26621841
x1,51:31614142,26621841
k1,51:31614142,26621841:0
)
(1,52:8865054,27408273:22749088,451360,127400
x1,52:9411054,27408273
k1,51:9651193,27408273:240139
x1,51:10599413,27408273
x1,51:11327413,27408273
x1,51:11691413,27408273
x1,51:12457633,27408273
k1,51:12697771,27408273:240138
x1,51:14919991,27408273
k1,51:15160130,27408273:240139
x1,51:17052930,27408273
x1,51:18184970,27408273
k1,51:18425109,27408273:240139
x1,51:19626309,27408273
x1,51:21009509,27408273
k1,51:21249647,27408273:240138
x1,51:22123247,27408273
x1,51:23324447,27408273
x1,51:24001487,27408273
k1,51:24241626,27408273:240139
x1,51:25335446,27408273
x1,51:26247266,27408273
x1,51:27011666,27408273
x1,51:27139066,27408273
k1,51:27379205,27408273:240139
x1,51:28289205,27408273
k1,51:28529343,27408273:240138
x1,51:28893343,27408273
x1,51:29715983,27408273
k1,51:29956122,27408273:240139
x1,51:30684122,27408273
x1,51:31048122,27408273
x1,51:31614142,27408273
k1,51:31614142,27408273:0
)
(1,52:8865054,28194705:22749088,491400,163800
x1,52:9229054,28194705
x1,51:10666854,28194705
k1,51:10974716,28194705:307862
x1,51:11666316,28194705
k1,51:11974178,28194705:307862
x1,51:12993378,28194705
x1,51:14378398,28194705
k1,51:14686259,28194705:307861
x1,51:14977459,28194705
x1,51:15942059,28194705
x1,51:16724659,28194705
x1,51:16997659,28194705
k1,51:17305521,28194705:307862
x1,51:18506721,28194705
x1,51:19889921,28194705
k1,51:20197783,28194705:307862
x1,51:21071383,28194705
x1,51:22272583,28194705
x1,51:22509183,28194705
k1,51:22817045,28194705:307862
x1,51:23508645,28194705
x1,51:25292245,28194705
k1,51:25600107,28194705:307862
x1,51:26040547,28194705
k1,51:26348409,28194705:307862
x1,51:26712409,28194705
x1,51:27040009,28194705
k1,51:27347870,28194705:307861
x1,51:30614770,28194705
k1,51:30922542,28194705:307772
x1,51:31614142,28194705
k1,51:31614142,28194705:0
)
(1,52:8865054,28981137:22749088,533465,127431
x1,52:9502054,28981137
x1,52:9866054,28981137
x1,52:10432074,28981137
x1,52:10614074,28981137
x1,52:11815274,28981137
x1,52:12051874,28981137
k1,51:12254456,28981137:202582
x1,51:13310056,28981137
k1,51:13512638,28981137:202582
x1,51:13953078,28981137
k1,51:14155660,28981137:202582
x1,51:14847260,28981137
k1,51:15049842,28981137:202582
x1,51:15959842,28981137
k1,51:16162424,28981137:202582
x1,51:16981424,28981137
x1,51:17436424,28981137
k1,51:17639006,28981137:202582
$1,51:17639006,28981137
x1,51:18476413,28981137
k1,51:18590402,28981137:113989
x1,51:19100128,28981137
k1,51:19214117,28981137:113989
x1,51:19869479,28981137
(1,51:19869479,28743312:964839,295640,54614
x1,51:20801550,28743312
)
x1,51:21229204,28981137
(1,51:21229204,29079440:451084,313481,0
x1,51:21625187,29079440
)
$1,51:21680288,28981137
x1,51:21862288,28981137
k1,51:22064870,28981137:202582
x1,51:22492570,28981137
x1,51:23022190,28981137
k1,51:23224772,28981137:202582
x1,51:23552372,28981137
k1,51:23754954,28981137:202582
x1,51:24302774,28981137
x1,51:25594974,28981137
k1,51:25797556,28981137:202582
x1,51:26325356,28981137
k1,51:26527938,28981137:202582
x1,51:27437938,28981137
x1,51:28367958,28981137
k1,51:28570540,28981137:202582
x1,51:29626140,28981137
k1,51:29828722,28981137:202582
x1,51:30465722,28981137
x1,51:30829722,28981137
x1,51:31395742,28981137
x1,51:31614142,28981137
k1,52:31614142,28981137:0
)
(1,52:8865054,29767569:22749088,491400,163800
x1,52:9047054,29767569
x1,52:10248254,29767569
x1,52:10484854,29767569
k1,51:10757752,29767569:272898
x1,51:11285552,29767569
k1,51:11558451,29767569:272899
x1,51:12577651,29767569
x1,51:13962671,29767569
k1,51:14235569,29767569:272898
x1,51:15291169,29767569
x1,51:16130189,29767569
x1,51:17331389,29767569
x1,51:18714589,29767569
k1,51:18987487,29767569:272898
x1,51:19935707,29767569
x1,51:20299707,29767569
x1,51:20865727,29767569
x1,51:21852167,29767569
k1,51:22125066,29767569:272899
x1,51:22965906,29767569
k1,51:23238804,29767569:272898
x1,51:23930404,29767569
k1,51:24039607,29767569:0
x1,51:24731207,29767569
k1,51:25004105,29767569:272898
x1,51:25240705,29767569
x1,51:25604705,29767569
x1,51:26389125,29767569
x1,51:27007925,29767569
x1,51:28136325,29767569
k1,51:28409224,29767569:272899
x1,51:28937024,29767569
k1,51:29209922,29767569:272898
x1,51:30229122,29767569
x1,51:31614142,29767569
k1,51:31614142,29767569:0
)
(1,52:8865054,30554001:22749088,451360,127400
x1,52:10066254,30554001
x1,52:11449454,30554001
k1,51:11662303,30554001:212849
x1,51:12535903,30554001
x1,51:13737103,30554001
x1,51:14232143,30554001
k1,51:14444992,30554001:212849
x1,51:15718992,30554001
k1,51:15931840,30554001:212848
x1,51:16259440,30554001
k1,51:16472289,30554001:212849
x1,51:17673489,30554001
x1,51:19056689,30554001
k1,51:19269538,30554001:212849
x1,51:20470738,30554001
k1,51:20683587,30554001:212849
x1,51:21229587,30554001
x1,51:22798427,30554001
k1,51:23011276,30554001:212849
x1,51:24030476,30554001
x1,51:25415496,30554001
k1,51:25628344,30554001:212848
x1,51:26796784,30554001
k1,51:27009633,30554001:212849
x1,51:28065233,30554001
k1,51:28278082,30554001:212849
x1,51:29664922,30554001
x1,51:30356522,30554001
x1,51:30684122,30554001
x1,51:31614142,30554001
k1,51:31614142,30554001:0
)
(1,52:8865054,31340433:22749088,451360,127400
x1,52:9776874,31340433
x1,52:10617714,31340433
x1,52:11931754,31340433
k1,51:12129315,31340433:197561
x1,51:12966515,31340433
k1,51:13164076,31340433:197561
x1,51:14183276,31340433
x1,51:15420876,31340433
x1,51:16403676,31340433
k1,51:16601236,31340433:197560
x1,51:17147236,31340433
k1,51:17344797,31340433:197561
x1,51:18655197,31340433
x1,51:19000997,31340433
k1,51:19198558,31340433:197561
x1,51:20217758,31340433
x1,51:20911178,31340433
x1,51:21861218,31340433
k1,51:22058779,31340433:197561
x1,51:22677579,31340433
x1,51:23041579,31340433
x1,51:23369179,31340433
x1,51:24153599,31340433
k1,51:24351160,31340433:197561
x1,51:24933560,31340433
k1,51:25131120,31340433:197560
x1,51:26261340,31340433
x1,51:26716340,31340433
x1,51:28791140,31340433
k1,51:28988701,31340433:197561
x1,51:30815981,31340433
k1,51:31013542,31340433:197561
x1,51:31614142,31340433
k1,51:31614142,31340433:0
)
(1,52:8865054,32126865:22749088,451360,127400
x1,52:9813274,32126865
x1,52:10541274,32126865
x1,52:10905274,32126865
x1,52:11853494,32126865
k1,51:12102197,32126865:248703
x1,51:13270637,32126865
k1,51:13519340,32126865:248703
x1,51:14431160,32126865
x1,51:15272000,32126865
x1,51:16404040,32126865
k1,51:16652742,32126865:248702
x1,51:17635542,32126865
k1,51:17884245,32126865:248703
x1,51:18248245,32126865
x1,51:18557645,32126865
k1,51:18806348,32126865:248703
x1,51:19352348,32126865
x1,51:21026748,32126865
k1,51:21275451,32126865:248703
x1,51:21639451,32126865
x1,51:21967051,32126865
k1,51:22215754,32126865:248703
x1,51:23234954,32126865
x1,51:24619974,32126865
k1,51:24868676,32126865:248702
x1,51:25050676,32126865
x1,51:25414676,32126865
x1,51:26199096,32126865
x1,51:26817896,32126865
x1,51:27946296,32126865
k1,51:28194999,32126865:248703
x1,51:29468999,32126865
k1,51:29717702,32126865:248703
x1,51:30594942,32126865
x1,51:31614142,32126865
k1,51:31614142,32126865:0
)
(1,52:8865054,32913297:22749088,491400,163800
x1,52:10066254,32913297
x1,52:11449454,32913297
g1,51:11667854,32913297
x1,51:13051054,32913297
g1,51:13269454,32913297
x1,51:14470654,32913297
g1,51:14689054,32913297
x1,51:15129494,32913297
g1,51:15347894,32913297
x1,51:15875694,32913297
g1,51:16094094,32913297
x1,51:16678314,32913297
x1,51:17590134,32913297
g1,51:17808534,32913297
x1,51:18336334,32913297
g1,51:18554734,32913297
$1,51:18554734,32913297
x1,51:18949620,32913297
$1,51:18949620,32913297
x1,51:19463770,32913297
g1,51:19682170,32913297
x1,51:20228170,32913297
g1,51:20446570,32913297
x1,51:21394790,32913297
g1,51:21613190,32913297
x1,51:23656140,32913297
g1,51:23874540,32913297
x1,51:24748140,32913297
k1,52:31614142,32913297:6866002
g1,52:31614142,32913297
)
(1,54:8865054,33699729:22749088,451360,127400
h1,53:8865054,33699729:983040,0,0
x1,53:10321294,33699729
x1,53:10594294,33699729
k1,53:10855033,33699729:260739
x1,53:12442073,33699729
k1,53:12702811,33699729:260738
x1,53:15365471,33699729
k1,53:15626210,33699729:260739
x1,53:19049630,33699729
k1,53:19310369,33699729:260739
x1,53:21568989,33699729
k1,53:21829727,33699729:260738
x1,53:25400567,33699729
k1,53:25661306,33699729:260739
x1,53:27270186,33699729
k1,53:27530925,33699729:260739
x1,53:27967725,33699729
k1,53:28228463,33699729:260738
x1,53:28668903,33699729
k1,53:28929642,33699729:260739
x1,53:31614142,33699729
k1,53:31614142,33699729:0
)
(1,54:8865054,34486161:22749088,451360,127400
x1,54:9447454,34486161
k1,53:9682978,34486161:235524
x1,53:11393778,34486161
x1,53:11721378,34486161
k1,53:11956903,34486161:235525
x1,53:12866903,34486161
k1,53:13102427,34486161:235524
x1,53:13575627,34486161
x1,53:13885027,34486161
x1,53:14212627,34486161
x1,53:14485627,34486161
k1,53:14721151,34486161:235524
x1,53:15703951,34486161
x1,53:16031551,34486161
x1,53:16559351,34486161
k1,53:16794876,34486161:235525
x1,53:19053496,34486161
x1,53:19399296,34486161
k1,53:19634820,34486161:235524
x1,53:20836020,34486161
k1,53:21071545,34486161:235525
x1,53:23037145,34486161
x1,53:23532185,34486161
k1,53:23767709,34486161:235524
x1,53:24552129,34486161
k1,53:24787653,34486161:235524
x1,53:28211073,34486161
k1,53:28446598,34486161:235525
x1,53:28974398,34486161
k1,53:29209922,34486161:235524
x1,53:31614142,34486161
k1,53:31614142,34486161:0
)
(1,54:8865054,35272593:22749088,451360,127400
x1,54:12184734,35272593
k1,53:12374924,35272593:190190
x1,53:15374284,35272593
x1,53:15501684,35272593
k1,53:15691874,35272593:190190
x1,53:16601874,35272593
k1,53:16792063,35272593:190189
x1,53:17265263,35272593
x1,53:17574663,35272593
x1,53:17902263,35272593
x1,53:18175263,35272593
k1,53:18365453,35272593:190190
x1,53:19348253,35272593
x1,53:19675853,35272593
x1,53:20203653,35272593
k1,53:20393843,35272593:190190
x1,53:23220303,35272593
k1,53:23410493,35272593:190190
x1,53:23883693,35272593
x1,53:24451533,35272593
k1,53:24641723,35272593:190190
x1,53:25642723,35272593
x1,53:26789323,35272593
x1,53:27462723,35272593
k1,53:27652913,35272593:190190
x1,53:28437333,35272593
k1,53:28627522,35272593:190189
x1,53:29537522,35272593
k1,53:29727712,35272593:190190
x1,53:30896152,35272593
k1,53:31086342,35272593:190190
x1,53:31614142,35272593
k1,53:31614142,35272593:0
)
(1,54:8865054,36059025:22749088,491400,163800
x1,54:9210854,36059025
x1,53:11067254,36059025
k1,53:11248253,36059025:180999
x1,53:13652473,36059025
k1,53:13833472,36059025:180999
x1,53:16971152,36059025
k1,53:17152150,36059025:180998
x1,53:18939390,36059025
k1,53:19120389,36059025:180999
x1,53:19904809,36059025
k1,53:20085808,36059025:180999
x1,53:20413408,36059025
k1,53:20594407,36059025:180999
x1,53:22871227,36059025
k1,53:23052226,36059025:180999
x1,53:25456446,36059025
k1,53:25637444,36059025:180998
x1,53:28775124,36059025
k1,53:28956123,36059025:180999
x1,53:29502123,36059025
k1,53:29683122,36059025:180999
x1,53:31614142,36059025
k1,53:31614142,36059025:0
)
(1,54:8865054,36845457:22749088,491400,163800
x1,54:9556654,36845457
k1,53:9665857,36845457:0
x1,53:10175457,36845457
k1,53:10435034,36845457:259577
x1,53:11490634,36845457
k1,53:11750211,36845457:259577
x1,53:14098011,36845457
x1,53:14371011,36845457
k1,53:14630588,36845457:259577
x1,53:17034808,36845457
k1,53:17294385,36845457:259577
x1,53:20432065,36845457
k1,53:20691642,36845457:259577
x1,53:21565242,36845457
k1,53:21824820,36845457:259578
x1,53:22425420,36845457
k1,53:22684997,36845457:259577
x1,53:23744237,36845457
k1,53:24003814,36845457:259577
x1,53:25059414,36845457
x1,53:25625434,36845457
k1,53:25885011,36845457:259577
x1,53:26358211,36845457
x1,53:26631211,36845457
k1,53:26890788,36845457:259577
x1,53:28801788,36845457
k1,53:29061365,36845457:259577
x1,53:29971365,36845457
k1,53:30230942,36845457:259577
x1,53:30704142,36845457
x1,53:31013542,36845457
x1,53:31341142,36845457
x1,53:31614142,36845457
k1,53:31614142,36845457:0
)
(1,54:8865054,37631889:22749088,451360,127400
x1,54:9847854,37631889
x1,53:10175454,37631889
x1,53:10703254,37631889
g1,53:10921654,37631889
x1,53:13180274,37631889
x1,53:13526074,37631889
g1,53:13744474,37631889
x1,53:14326874,37631889
g1,53:14545274,37631889
x1,53:15455274,37631889
g1,53:15673674,37631889
x1,53:16842114,37631889
g1,53:17060514,37631889
x1,53:17588314,37631889
g1,53:17806714,37631889
x1,53:20210934,37631889
g1,53:20429334,37631889
x1,53:23852754,37631889
g1,53:24071154,37631889
x1,53:24617154,37631889
g1,53:24835554,37631889
x1,53:25163154,37631889
g1,53:25381554,37631889
x1,53:27965954,37631889
g1,53:28184354,37631889
x1,53:29567554,37631889
k1,54:31614142,37631889:2046588
g1,54:31614142,37631889
)
(1,55:8865054,39470752:22749088,542724,152880
(1,55:8865054,39470752:1326780,509964,0
g1,55:8865054,39470752
x1,55:9307314,39470752
g1,55:10191834,39470752
)
x1,55:13663026,39470752
k1,55:13980026,39470752:317000
x1,55:18203609,39470752
k1,55:18520609,39470752:317000
x1,55:19257709,39470752
k1,55:19574710,39470752:317001
x1,55:20004685,39470752
k1,55:20321685,39470752:317000
x1,55:23808804,39470752
k1,55:24125804,39470752:317000
x1,55:25757888,39470752
k1,55:26074888,39470752:317000
x1,55:26811988,39470752
k1,55:27128989,39470752:317001
x1,55:28367953,39470752
k1,55:28684953,39470752:317000
x1,55:29323773,39470752
x1,55:29729178,39470752
x1,55:30171438,39470752
x1,55:30550452,39470752
k1,55:31614142,39470752:1063690
)
(1,55:10191834,40388256:21422308,542724,152880
x1,55:11506329,40388256
x1,55:11948589,40388256
x1,55:12671583,40388256
g1,55:12966423,40388256
x1,55:16784691,40388256
k1,55:31614142,40388256:14829451
g1,55:31614142,40388256
)
(1,57:8865054,41702832:22749088,451360,127400
x1,57:11396674,41702832
k1,56:11621609,41702832:224935
x1,56:14759289,41702832
k1,56:14984225,41702832:224936
x1,56:15530225,41702832
k1,56:15755160,41702832:224935
x1,56:16082760,41702832
k1,56:16307695,41702832:224935
x1,56:18548115,41702832
k1,56:18773050,41702832:224935
x1,56:21357450,41702832
k1,56:21582386,41702832:224936
x1,56:22783586,41702832
k1,56:23008521,41702832:224935
x1,56:23883941,41702832
k1,56:24108876,41702832:224935
x1,56:26116336,41702832
x1,56:26789736,41702832
k1,56:27014671,41702832:224935
x1,56:27378671,41702832
x1,56:27706271,41702832
k1,56:27931207,41702832:224936
x1,56:28841207,41702832
k1,56:29066142,41702832:224935
x1,56:30285542,41702832
x1,56:31614142,41702832
k1,56:31614142,41702832:0
)
(1,57:8865054,42489264:22749088,451360,127400
x1,57:9738654,42489264
x1,56:10302854,42489264
x1,56:11322054,42489264
g1,56:11540454,42489264
x1,56:13098374,42489264
g1,56:13316774,42489264
x1,56:15773774,42489264
k1,57:31614142,42489264:15840368
g1,57:31614142,42489264
)
(1,59:14928672,43608196:16685470,491520,187504
(1,59:14928672,43608196:10621852,491520,187504
x1,59:15748615,43608196
(1,59:15785023,43337603:351425,197518,89201
x1,59:16103680,43337603
)
x1,59:16484381,43608196
(1,59:16484381,43706499:351425,197518,89201
x1,59:16803038,43706499
)
g1,59:16981438,43608196
x1,59:17491164,43608196
g1,59:17636796,43608196
x1,59:18212211,43608196
(1,59:18212211,43706499:218188,303558,0
x1,59:18397631,43706499
)
x1,59:19008998,43608196
(1,59:19008998,43706499:218188,303558,0
x1,59:19194418,43706499
)
x1,59:20111468,43608196
g1,59:20257100,43608196
x1,59:20766826,43608196
g1,59:20912458,43608196
x1,59:21307344,43608196
(1,59:21307344,43706499:218188,303558,0
x1,59:21492764,43706499
)
x1,59:22105568,43608196
x1,59:22709100,43608196
x1,59:23064522,43608196
(1,59:23064522,43706499:218188,303558,0
x1,59:23249942,43706499
)
x1,59:24166992,43608196
g1,59:24349032,43608196
x1,59:24858758,43608196
g1,59:25040798,43608196
x1,59:25550524,43608196
)
(1,59:30776942,43608196:837200,491400,163800
(1,59:30776942,43608196:837200,491400,163800
x1,59:31614142,43608196
)
)
)
]
(1,61:8865054,45574276:22749088,0,0
h1,61:8865054,45574276:22749088,0,0
)
]
]
!26741
}1
!10
{2
[1,103:4736286,45574276:26877856,40837990,0
(1,103:4736286,4736286:0,0,0
[1,103:0,4736286:0,0,0
(1,103:0,0:0,0,0
g1,103:0,0
)
]
)
[1,103:8865054,45574276:22749088,39789414,0
[1,103:8865054,6571294:22749088,786432,0
(1,103:8865054,6571294:22749088,406224,114660
(1,103:8865054,6571294:22749088,406224,114660
(1,103:8865054,6571294:0,379288,0
x1,103:9168084,6571294
k1,103:8865054,6571294:-303030
)
g1,103:11039271,6571294
(1,40:11039271,6571294:4032070,406224,114660
x1,40:11662074,6571294
g1,40:11864094,6571294
x1,40:12276506,6571294
x1,40:12899400,6571294
x1,40:13219265,6571294
x1,40:13522294,6571294
g1,40:13724314,6571294
x1,40:14229591,6571294
g1,40:14431611,6571294
x1,40:15071341,6571294
)
k1,103:31614142,6571294:16542801
)
)
]
[1,103:8865054,43608196:22749088,35988326,0
(1,61:8865054,8275230:22749088,491400,163800
x1,61:10541274,8275230
k1,60:10741496,8275230:200222
$1,60:10741496,8275230
x1,60:10967276,8275230
k1,60:11149316,8275230:182040
x1,60:11659042,8275230
k1,60:11841082,8275230:182040
x1,60:12350808,8275230
k1,60:12460032,8275230:109224
x1,60:12969758,8275230
k1,60:13078982,8275230:109224
x1,60:13406663,8275230
$1,60:13406663,8275230
k1,60:13606885,8275230:200222
x1,60:14262085,8275230
x1,60:14607885,8275230
x1,60:15701705,8275230
x1,60:16833745,8275230
k1,60:17033966,8275230:200221
x1,60:18053166,8275230
x1,60:19438186,8275230
k1,60:19638408,8275230:200222
x1,60:20770448,8275230
x1,60:21556688,8275230
x1,60:21829688,8275230
k1,60:22029910,8275230:200222
x1,60:23857190,8275230
k1,60:24057412,8275230:200222
x1,60:24658012,8275230
k1,60:24858234,8275230:200222
x1,60:25549834,8275230
k1,60:25659037,8275230:0
x1,60:26678237,8275230
k1,60:26878458,8275230:200221
x1,60:28207058,8275230
x1,60:29335458,8275230
k1,60:29535680,8275230:200222
x1,60:30118080,8275230
h1,60:30118080,8275230:0,0,0
x1,60:30372880,8275230
k1,60:30573102,8275230:200222
x1,60:31046302,8275230
x1,60:31614142,8275230
k1,60:31614142,8275230:0
)
(1,61:8865054,9061662:22749088,451360,127400
x1,61:9978894,9061662
x1,60:10615894,9061662
k1,60:10876973,9061662:261079
x1,60:11422973,9061662
k1,60:11684052,9061662:261079
x1,60:12594052,9061662
k1,60:12855130,9061662:261078
x1,60:14383930,9061662
k1,60:14645009,9061662:261079
x1,60:15118209,9061662
x1,60:15427609,9061662
x1,60:15755209,9061662
x1,60:16028209,9061662
k1,60:16289288,9061662:261079
x1,60:16980888,9061662
x1,60:17929108,9061662
x1,60:18256708,9061662
x1,60:18438708,9061662
x1,60:19312308,9061662
x1,60:20622708,9061662
k1,60:20883787,9061662:261079
x1,60:21356987,9061662
x1,60:21629987,9061662
k1,60:21891066,9061662:261079
x1,60:22509866,9061662
x1,60:23856666,9061662
x1,60:24093266,9061662
k1,60:24354344,9061662:261078
x1,60:25138764,9061662
k1,60:25399843,9061662:261079
x1,60:25763843,9061662
x1,60:26109643,9061662
x1,60:26655643,9061662
x1,60:27019643,9061662
x1,60:28475643,9061662
k1,60:28736722,9061662:261079
x1,60:29464722,9061662
x1,60:29828722,9061662
x1,60:30431142,9061662
x1,60:31377542,9061662
x1,60:31614142,9061662
k1,60:31614142,9061662:0
)
(1,61:8865054,9848094:22749088,491400,163800
x1,61:9520254,9848094
x1,61:10139054,9848094
x1,61:11050874,9848094
x1,61:12288474,9848094
k1,60:12573635,9848094:285161
x1,60:12864835,9848094
x1,60:14342675,9848094
k1,60:14627835,9848094:285160
x1,60:15173835,9848094
k1,60:15458996,9848094:285161
x1,60:16478196,9848094
x1,60:17863216,9848094
k1,60:18148377,9848094:285161
x1,60:18734417,9848094
x1,60:19389617,9848094
x1,60:19899217,9848094
x1,60:21286057,9848094
k1,60:21571218,9848094:285161
x1,60:22153618,9848094
k1,60:22438778,9848094:285160
x1,60:23639978,9848094
k1,60:23925139,9848094:285161
x1,60:24729579,9848094
x1,60:26698819,9848094
k1,60:26983980,9848094:285161
x1,60:27457180,9848094
x1,60:27730180,9848094
k1,60:28015341,9848094:285161
x1,60:29129181,9848094
x1,60:29402181,9848094
k1,60:29687341,9848094:285160
x1,60:30269741,9848094
h1,60:30269741,9848094:0,0,0
x1,60:30524541,9848094
k1,60:30809702,9848094:285161
x1,60:31395742,9848094
x1,60:31614142,9848094
k1,61:31614142,9848094:0
)
(1,61:8865054,10634526:22749088,451360,127400
x1,61:10033494,10634526
x1,61:10907094,10634526
k1,60:11150787,10634526:243693
x1,60:12351987,10634526
k1,60:12595681,10634526:243694
x1,60:13178081,10634526
k1,60:13421774,10634526:243693
x1,60:14149774,10634526
x1,60:15096174,10634526
k1,60:15339867,10634526:243693
x1,60:16213467,10634526
x1,60:17414667,10634526
x1,60:17651267,10634526
k1,60:17894961,10634526:243694
$1,60:17894961,10634526
x1,60:18131619,10634526
k1,60:18355824,10634526:224205
x1,60:18865550,10634526
k1,60:19089754,10634526:224204
x1,60:19417435,10634526
$1,60:19417435,10634526
k1,60:19661129,10634526:243694
x1,60:20680329,10634526
x1,60:22065349,10634526
k1,60:22309042,10634526:243693
x1,60:22782242,10634526
x1,60:23091642,10634526
x1,60:23419242,10634526
x1,60:23692242,10634526
k1,60:23935935,10634526:243693
x1,60:25155335,10634526
x1,60:26283735,10634526
k1,60:26527429,10634526:243694
x1,60:26955129,10634526
x1,60:28578569,10634526
k1,60:28822262,10634526:243693
x1,60:30283722,10634526
x1,60:31614142,10634526
k1,60:31614142,10634526:0
)
(1,61:8865054,11420958:22749088,451360,127400
x1,61:9305494,11420958
g1,60:9523894,11420958
x1,60:10179094,11420958
x1,60:11531354,11420958
x1,60:12204754,11420958
g1,60:12423154,11420958
x1,60:12787154,11420958
x1,60:13114754,11420958
g1,60:13333154,11420958
x1,60:13660754,11420958
g1,60:13879154,11420958
x1,60:15343344,11420958
x1,60:16475384,11420958
g1,60:16693784,11420958
x1,60:17166984,11420958
x1,60:17476384,11420958
x1,60:17803984,11420958
x1,60:18076984,11420958
g1,60:18295384,11420958
x1,60:19278184,11420958
x1,60:19605784,11420958
x1,60:20133584,11420958
k1,61:31614142,11420958:11480558
g1,61:31614142,11420958
)
(1,64:10102080,12983407:21512062,976821,712513
(1,64:10102080,12983407:19437836,976821,712513
x1,64:10425816,12983407
(1,64:10425816,13081710:218188,303558,0
x1,64:10611236,13081710
)
x1,64:11410640,12983407
g1,64:11519864,12983407
x1,64:12102408,12983407
g1,64:12284448,12983407
x1,64:12794174,12983407
g1,64:12976214,12983407
x1,64:13297069,12983407
(1,64:13297069,13081710:218188,303558,0
x1,64:13482489,13081710
)
x1,64:14281893,12983407
g1,64:14391117,12983407
x1,64:14720845,12983407
(1,64:14720845,13081710:294003,295640,0
x1,64:14982080,13081710
)
x1,64:15644877,12983407
[1,64:15644877,13166083:442369,747014,0
(1,64:15644877,12703059:442369,283990,54614
x1,64:16054478,12703059
)
(1,64:15644877,13166083:218188,303558,0
x1,64:15830297,13166083
)
]
x1,64:17108745,12983407
g1,62:17290785,12983407
g1,62:17472825,12983407
g1,62:17654865,12983407
g1,64:17764089,12983407
x1,64:18084944,12983407
(1,64:18084944,13081710:218188,303558,0
x1,64:18270364,13081710
)
x1,64:19069768,12983407
g1,64:19178992,12983407
x1,64:19508720,12983407
(1,64:19508720,13081710:294003,295640,0
x1,64:19769955,13081710
)
x1,64:20057586,12983407
g1,64:20239626,12983407
x1,64:20749352,12983407
g1,64:20931392,12983407
(1,64:20931392,12983407:2907530,865699,712513
(1,64:20931392,12983407:2907530,865699,712513
h1,64:20931392,12983407:78643,0,0
[1,64:21010035,12983407:2750244,865699,712513
(1,64:21010035,12540051:2750244,422343,0
k1,64:22221317,12540051:1211282
x1,64:22548998,12540051
k1,64:23760279,12540051:1211281
)
(1,64:21010035,13444702:2750244,533390,251217
x1,64:21966152,13444702
x1,64:22364146,13444702
[1,64:22364146,13606718:317516,646982,89201
(1,64:22387659,13255376:294003,295640,0
x1,64:22648894,13255376
)
(1,64:22364146,13606718:302930,197518,89201
x1,64:22634308,13606718
)
]
x1,64:22936525,13444702
(1,64:22936525,13255376:823754,344064,114688
x1,64:23727511,13255376
)
)
]
h1,64:23760279,12983407:78643,0,0
)
)
g1,64:23948146,12983407
(1,64:23948146,12983407:1001247,282168,127431
x1,64:24949393,12983407
)
g1,64:25058617,12983407
(1,64:25058617,12983407:4190030,976821,700762
(1,64:25058617,12059341:482420,26213,1546666
x1,64:25541037,12059341
)
x1,64:26050763,12983407
(1,64:26050763,12983407:2715464,976821,700762
(1,64:26050763,12983407:2715464,976821,700762
h1,64:26050763,12983407:78643,0,0
[1,64:26129406,12983407:2558178,976821,700762
(1,64:26129406,12540051:2558178,533465,163840
x1,64:26713997,12540051
g1,64:26859629,12540051
x1,64:27369355,12540051
g1,64:27514987,12540051
x1,64:27844715,12540051
(1,64:27844715,12638354:294003,295640,0
x1,64:28105950,12638354
)
x1,64:28393581,12540051
(1,64:28393581,12302226:294003,295640,0
x1,64:28654816,12302226
)
)
(1,64:26129406,13432951:2558178,484966,251217
k1,64:26898656,13432951:769250
x1,64:27600818,13432951
[1,64:27600818,13594967:317516,646982,89201
(1,64:27624331,13243625:294003,295640,0
x1,64:27885566,13243625
)
(1,64:27600818,13594967:302930,197518,89201
x1,64:27870980,13594967
)
]
k1,64:28687584,13432951:769250
)
]
h1,64:28687584,12983407:78643,0,0
)
)
(1,64:28766227,12059341:482420,26213,1546666
x1,64:29248647,12059341
)
)
g1,64:29357871,12983407
x1,64:29539916,12983407
)
(1,64:30776942,12983407:837200,491400,163800
(1,64:30776942,12983407:837200,491400,163800
x1,64:31614142,12983407
)
)
)
(1,66:8865054,14605508:22749088,451360,187504
x1,66:10541274,14605508
k1,65:10835076,14605508:293802
$1,65:10835076,14605508
x1,65:11164804,14605508
(1,65:11164804,14703811:294003,295640,0
x1,65:11426039,14703811
)
$1,65:11458807,14605508
k1,65:11752609,14605508:293802
x1,65:12193049,14605508
k1,65:12486851,14605508:293802
x1,65:13396851,14605508
k1,65:13690653,14605508:293802
x1,65:14018253,14605508
x1,65:14345853,14605508
x1,65:15821873,14605508
k1,65:16115675,14605508:293802
x1,65:16588875,14605508
x1,65:16898275,14605508
x1,65:17225875,14605508
x1,65:17498875,14605508
k1,65:17792677,14605508:293802
x1,65:18775477,14605508
x1,65:19103077,14605508
x1,65:19630877,14605508
k1,65:19924679,14605508:293802
x1,65:21999479,14605508
x1,65:23328079,14605508
k1,65:23621881,14605508:293802
$1,65:23621881,14605508
x1,65:23996362,14605508
(1,65:23996362,14703811:302930,197518,89201
x1,65:24266524,14703811
)
$1,65:24299292,14605508
k1,65:24593094,14605508:293802
x1,65:25033534,14605508
k1,65:25327336,14605508:293802
x1,65:25800536,14605508
x1,65:26109936,14605508
x1,65:26437536,14605508
x1,65:26710536,14605508
k1,65:27004338,14605508:293802
x1,65:27987138,14605508
x1,65:28314738,14605508
x1,65:28842538,14605508
k1,65:29136340,14605508:293802
x1,65:30774340,14605508
k1,65:31068142,14605508:293802
x1,65:31614142,14605508
k1,65:31614142,14605508:0
)
(1,66:8865054,15391940:22749088,564338,182676
x1,66:10939854,15391940
x1,65:12086454,15391940
g1,65:12304854,15391940
x1,65:13837294,15391940
g1,65:14055694,15391940
x1,65:15111294,15391940
g1,65:15329694,15391940
$1,65:15329694,15391940
x1,65:15704860,15391940
[1,65:15704860,15574616:442369,747014,0
(1,65:15704860,15111592:442369,283990,54614
x1,65:16114461,15111592
)
(1,65:15704860,15574616:218188,303558,0
x1,65:15890280,15574616
)
]
$1,65:16147229,15391940
g1,65:16365629,15391940
x1,65:16806069,15391940
g1,65:17024469,15391940
x1,65:17352069,15391940
g1,65:17570469,15391940
x1,65:18717069,15391940
x1,65:20791869,15391940
g1,65:21010269,15391940
x1,65:23270709,15391940
g1,65:23489109,15391940
x1,65:24016909,15391940
g1,65:24235309,15391940
x1,65:24581109,15391940
x1,65:26437509,15391940
g1,65:26655909,15391940
x1,65:28213829,15391940
g1,65:28432229,15391940
x1,65:31071229,15391940
k1,66:31614142,15391940:542913
g1,66:31614142,15391940
)
(1,68:8865054,16178372:22749088,451360,127400
h1,67:8865054,16178372:983040,0,0
x1,67:10976494,16178372
k1,67:11134729,16178372:158235
x1,67:12303169,16178372
x1,67:14001229,16178372
k1,67:14159465,16178372:158236
x1,67:16345285,16178372
k1,67:16503520,16178372:158235
x1,67:17287940,16178372
k1,67:17446175,16178372:158235
x1,67:20108835,16178372
k1,67:20267070,16178372:158235
x1,67:20813070,16178372
x1,67:23344690,16178372
k1,67:23502926,16178372:158236
x1,67:24776926,16178372
k1,67:24935161,16178372:158235
x1,67:25262761,16178372
k1,67:25420996,16178372:158235
x1,67:28005396,16178372
k1,67:28163631,16178372:158235
x1,67:29364831,16178372
k1,67:29523067,16178372:158236
x1,67:29963507,16178372
k1,67:30121742,16178372:158235
x1,67:30977142,16178372
x1,67:31614142,16178372
k1,67:31614142,16178372:0
)
(1,68:8865054,16964804:22749088,491400,163800
x1,68:9229054,16964804
x1,67:9556654,16964804
g1,67:9775054,16964804
x1,67:10685054,16964804
g1,67:10903454,16964804
x1,67:12122854,16964804
x1,67:13451454,16964804
g1,67:13669854,16964804
x1,67:16609154,16964804
g1,67:16827554,16964804
x1,67:17519154,16964804
k1,68:31614142,16964804:14094988
g1,68:31614142,16964804
)
(1,70:12714642,18697400:18899500,1110567,488525
(1,70:12714642,18697400:15049913,1110567,488525
x1,70:13198425,18697400
[1,70:13198425,18859416:317895,630127,0
(1,70:13236198,18426807:280122,197518,0
x1,70:13483552,18426807
)
(1,70:13198425,18859416:218188,303558,0
x1,70:13383845,18859416
)
]
x1,70:14355774,18697400
g1,70:14537814,18697400
x1,70:15047540,18697400
g1,70:15229580,18697400
x1,70:15739306,18697400
(1,70:15739306,18697400:12025249,1110567,488525
(1,70:15739306,17639259:655361,26213,1546666
x1,70:16394667,17639259
)
[1,70:16394667,18697400:11369888,1110567,366506
(1,70:16394667,18697400:11369888,839366,366506
x1,70:16970082,18697400
[1,70:16970082,18880076:294003,704050,0
(1,70:16970082,18471666:294003,295640,0
x1,70:17231317,18471666
)
(1,70:16970082,18880076:218188,303558,0
x1,70:17155502,18880076
)
]
g1,70:17409717,18697400
x1,70:17919443,18697400
g1,70:18065075,18697400
x1,70:18394803,18697400
(1,70:18394803,18508074:294003,295640,0
x1,70:18656038,18508074
)
g1,70:18834438,18697400
x1,70:19344164,18697400
g1,70:19489796,18697400
x1,70:19884682,18697400
[1,70:19884682,18880076:294003,704050,0
(1,70:19884682,18471666:294003,295640,0
x1,70:20145917,18471666
)
(1,70:19884682,18880076:218188,303558,0
x1,70:20070102,18880076
)
]
x1,70:20675781,18697400
(1,70:20708662,18508074:294003,295640,0
x1,70:20969897,18508074
)
g1,70:21148297,18697400
x1,70:21658023,18697400
g1,70:21803655,18697400
x1,70:22833422,18697400
(1,70:22833422,18795703:218188,303558,0
x1,70:23018842,18795703
)
(1,70:23051610,18697400:4712945,839366,366506
(1,70:23051610,17910460:655361,26213,1153446
x1,70:23706971,17910460
)
[1,70:23706971,18697400:4057584,839366,197695
(1,70:23706971,18697400:4057584,521374,197695
x1,70:24282386,18697400
[1,70:24282386,18880076:294003,704050,0
(1,70:24282386,18471666:294003,295640,0
x1,70:24543621,18471666
)
(1,70:24282386,18880076:218188,303558,0
x1,70:24467806,18880076
)
]
x1,70:25073485,18697400
(1,70:25106366,18508074:294003,295640,0
x1,70:25367601,18508074
)
g1,70:25546001,18697400
x1,70:26055727,18697400
g1,70:26201359,18697400
x1,70:26531087,18697400
(1,70:26531087,18508074:294003,295640,0
x1,70:26792322,18508074
)
x1,70:27322186,18697400
[1,70:27322186,18895095:442369,719069,0
(1,70:27355067,18471666:294003,295640,0
x1,70:27616302,18471666
)
(1,70:27322186,18895095:442369,318577,0
x1,70:27731787,18895095
)
]
)
]
)
)
]
)
)
(1,70:30776942,18697400:837200,491400,163800
(1,70:30776942,18697400:837200,491400,163800
x1,70:31614142,18697400
)
)
)
(1,72:8865054,20095513:22749088,451360,127400
x1,72:10541274,20095513
k1,71:10808691,20095513:267417
$1,71:10808691,20095513
x1,71:11115891,20095513
k1,71:11379643,20095513:263752
x1,71:11889369,20095513
k1,71:12153121,20095513:263752
x1,71:12990528,20095513
$1,71:12990528,20095513
x1,71:13172528,20095513
k1,71:13439945,20095513:267417
x1,71:14770365,20095513
k1,71:15037782,20095513:267417
x1,71:17622182,20095513
k1,71:17889598,20095513:267416
x1,71:19090798,20095513
k1,71:19358215,20095513:267417
$1,71:19358215,20095513
x1,71:19926021,20095513
$1,71:19957707,20095513
k1,71:20225124,20095513:267417
x1,71:20771124,20095513
k1,71:21038540,20095513:267416
x1,71:23222540,20095513
x1,71:24481980,20095513
k1,71:24749397,20095513:267417
x1,71:25295397,20095513
x1,71:25859597,20095513
k1,71:26127014,20095513:267417
x1,71:27934274,20095513
x1,71:29013534,20095513
k1,71:29280950,20095513:267416
$1,71:29280950,20095513
x1,71:29848756,20095513
(1,71:29848756,20193816:442369,318577,0
x1,71:30258357,20193816
)
$1,71:30291125,20095513
k1,71:30558542,20095513:267417
x1,71:31614142,20095513
k1,71:31614142,20095513:0
)
(1,72:8865054,20881945:22749088,451360,233018
x1,72:12286654,20881945
g1,71:12505054,20881945
$1,71:12505054,20881945
x1,71:13072860,20881945
(1,71:13072860,21000275:301284,344064,114688
x1,71:13341376,21000275
)
$1,71:13374144,20881945
g1,71:13592544,20881945
x1,71:15121344,20881945
x1,71:16486344,20881945
x1,71:16981384,20881945
g1,71:17199784,20881945
x1,71:18473784,20881945
g1,71:18692184,20881945
x1,71:19862444,20881945
x1,71:20717844,20881945
g1,71:20936244,20881945
x1,71:21518644,20881945
g1,71:21737044,20881945
x1,71:22647044,20881945
g1,71:22865444,20881945
x1,71:25269664,20881945
g1,71:25488064,20881945
x1,71:27562864,20881945
x1,71:28891464,20881945
k1,72:31614142,20881945:2722678
g1,72:31614142,20881945
)
(1,74:8865054,21668377:22749088,491400,163800
h1,73:8865054,21668377:983040,0,0
x1,73:11471534,21668377
k1,73:11659061,21668377:187527
x1,73:12241461,21668377
h1,73:12241461,21668377:0,0,0
x1,73:12678261,21668377
k1,73:12865788,21668377:187527
x1,73:13338988,21668377
x1,73:13611988,21668377
k1,73:13799514,21668377:187526
x1,73:16311114,21668377
k1,73:16498641,21668377:187527
x1,73:18902861,21668377
k1,73:19090388,21668377:187527
x1,73:19563588,21668377
x1,73:19872988,21668377
x1,73:20200588,21668377
x1,73:20473588,21668377
k1,73:20661115,21668377:187527
x1,73:21643915,21668377
x1,73:21971515,21668377
x1,73:22757755,21668377
k1,73:22945282,21668377:187527
x1,73:24585102,21668377
k1,73:24772628,21668377:187526
x1,73:25118428,21668377
x1,73:25901028,21668377
x1,73:27378868,21668377
k1,73:27566395,21668377:187527
x1,73:29531995,21668377
x1,73:30642195,21668377
k1,73:30829722,21668377:187527
x1,73:31614142,21668377
k1,73:31614142,21668377:0
)
(1,74:8865054,22454809:22749088,451360,127400
x1,74:11269274,22454809
g1,73:11487674,22454809
x1,73:12033674,22454809
x1,73:14565294,22454809
g1,73:14783694,22454809
x1,73:16057694,22454809
g1,73:16276094,22454809
x1,73:16603694,22454809
g1,73:16822094,22454809
x1,73:19406494,22454809
g1,73:19624894,22454809
x1,73:20826094,22454809
k1,74:31614142,22454809:10788048
g1,74:31614142,22454809
)
(1,76:11907476,24187326:19706666,1146889,819210
(1,76:11907476,24187326:16664244,1146889,819210
x1,76:12225144,24187326
[1,76:12225144,24349342:303635,630127,0
(1,76:12248657,23916733:280122,197518,0
x1,76:12496011,23916733
)
(1,76:12225144,24349342:218188,303558,0
x1,76:12410564,24349342
)
]
x1,76:13113370,24187326
(1,76:13113370,24285629:294003,295640,0
x1,76:13374605,24285629
)
x1,76:13662236,24187326
g1,76:13844276,24187326
x1,76:14354002,24187326
g1,76:14536042,24187326
(1,76:14536042,24187326:2182759,934876,576976
(1,76:14536042,24187326:2182759,934876,576976
h1,76:14536042,24187326:78643,0,0
[1,76:14614685,24187326:2025473,934876,576976
(1,76:14614685,23743970:2025473,491520,170585
x1,76:14962618,23743970
x1,76:15482809,23743970
[1,76:15482809,23914555:317895,605928,0
(1,76:15520582,23506145:280122,197518,0
x1,76:15767936,23506145
)
(1,76:15482809,23914555:218188,303558,0
x1,76:15668229,23914555
)
]
x1,76:16640158,23743970
)
(1,76:14614685,24636870:2025473,455111,127431
k1,76:15270387,24636870:655702
x1,76:15618320,24636870
x1,76:15984456,24636870
k1,76:16640158,24636870:655702
)
]
h1,76:16640158,24187326:78643,0,0
)
)
(1,75:16718801,24187326:218453,753670,425990
$1,75:16718801,24187326
(1,75:16718801,24187326:218453,753670,425990
[1,75:16718801,23433656:218453,0,1179660
(1,75:16718801,23433656:218453,0,393220
x1,75:16937254,23433656
)
(1,75:16718801,23826876:218453,0,393220
x1,75:16937254,23826876
)
(1,75:16718801,24220096:218453,0,393220
x1,75:16937254,24220096
)
]
v1,75:16937254,24187326:0,753664,0
h1,75:16937254,24187326:0,0,0
)
$1,75:16937254,24187326
)
(1,76:16937254,24646083:1231188,197518,89201
x1,76:17879898,24646083
(1,76:17879898,24711619:255776,211171,0
x1,76:18102906,24711619
)
)
g1,76:18350482,24187326
x1,76:18860208,24187326
g1,76:19042248,24187326
(1,76:19042248,24187326:2092421,725524,632221
(1,76:19042248,24187326:2092421,725524,632221
h1,76:19042248,24187326:78643,0,0
[1,76:19120891,24187326:1935135,725524,632221
(1,76:19120891,23743970:1935135,282168,127431
k1,76:19776593,23743970:655702
x1,76:20106321,23743970
(1,76:20106321,23842273:294003,295640,0
x1,76:20367556,23842273
)
k1,76:21056026,23743970:655702
)
(1,76:19120891,24636870:1935135,491520,182676
x1,76:19604674,24636870
[1,76:19604674,24819546:317895,605928,0
(1,76:19642447,24411136:280122,197518,0
x1,76:19889801,24411136
)
(1,76:19604674,24819546:218188,303558,0
x1,76:19790094,24819546
)
]
x1,76:20507160,24636870
(1,76:20507160,24735173:294003,295640,0
x1,76:20768395,24735173
)
x1,76:21056026,24636870
)
]
h1,76:21056026,24187326:78643,0,0
)
)
g1,76:21243893,24187326
(1,76:21243893,24187326:7036558,1146889,819210
(1,76:21243893,23066650:518828,26213,1939886
x1,76:21762721,23066650
)
x1,76:22090402,24187326
g1,76:22236034,24187326
x1,76:22745760,24187326
g1,76:22891392,24187326
(1,76:22891392,24187326:4870231,976821,740558
(1,76:22891392,24187326:4870231,976821,740558
h1,76:22891392,24187326:78643,0,0
[1,76:22970035,24187326:4712945,976821,740558
(1,76:22970035,23743970:4712945,533465,185604
k1,76:24396638,23743970:1426603
x1,76:25098724,23743970
(1,76:25098724,23842273:218188,303558,0
x1,76:25284144,23842273
)
x1,76:25814008,23743970
[1,76:25814008,23929574:442369,719069,0
(1,76:25846889,23506145:294003,295640,0
x1,76:26108124,23506145
)
(1,76:25814008,23929574:442369,318577,0
x1,76:26223609,23929574
)
]
k1,76:27682980,23743970:1426603
)
(1,76:22970035,24725993:4712945,610762,201890
(1,76:22970035,24167657:655361,26213,760226
x1,76:23625396,24167657
)
[1,76:23625396,24725993:4057584,610762,197695
(1,76:23625396,24725993:4057584,521374,197695
x1,76:24200811,24725993
[1,76:24200811,24908669:294003,704050,0
(1,76:24200811,24500259:294003,295640,0
x1,76:24462046,24500259
)
(1,76:24200811,24908669:218188,303558,0
x1,76:24386231,24908669
)
]
x1,76:24991910,24725993
(1,76:25024791,24536667:294003,295640,0
x1,76:25286026,24536667
)
g1,76:25464426,24725993
x1,76:25974152,24725993
g1,76:26119784,24725993
x1,76:26449512,24725993
[1,76:26449512,24900751:294003,696132,0
(1,76:26449512,24500259:294003,295640,0
x1,76:26710747,24500259
)
(1,76:26449512,24900751:294003,295640,0
x1,76:26710747,24900751
)
]
x1,76:27240611,24725993
[1,76:27240611,24923688:442369,719069,0
(1,76:27273492,24500259:294003,295640,0
x1,76:27534727,24500259
)
(1,76:27240611,24923688:442369,318577,0
x1,76:27650212,24923688
)
]
)
]
)
]
h1,76:27682980,24187326:78643,0,0
)
)
(1,76:27761623,23066650:518828,26213,1939886
x1,76:28280451,23066650
)
)
g1,76:28389675,24187326
x1,76:28571720,24187326
)
(1,76:30776942,24187326:837200,491400,163800
(1,76:30776942,24187326:837200,491400,163800
x1,76:31614142,24187326
)
)
)
(1,79:8865054,25916124:22749088,451360,127400
h1,78:8865054,25916124:983040,0,0
x1,78:11859194,25916124
x1,78:11986594,25916124
k1,78:12154647,25916124:168053
x1,78:12627847,25916124
x1,78:12900847,25916124
k1,78:13068900,25916124:168053
x1,78:15580500,25916124
k1,78:15748552,25916124:168052
x1,78:16658552,25916124
k1,78:16826605,25916124:168053
x1,78:20362865,25916124
k1,78:20530918,25916124:168053
x1,78:21058718,25916124
k1,78:21226771,25916124:168053
x1,78:23630991,25916124
k1,78:23799044,25916124:168053
x1,78:24490644,25916124
x1,78:24818244,25916124
x1,78:25748264,25916124
k1,78:25916316,25916124:168052
x1,78:26971916,25916124
k1,78:27139969,25916124:168053
x1,78:28308409,25916124
k1,78:28476462,25916124:168053
x1,78:31614142,25916124
k1,78:31614142,25916124:0
)
(1,79:8865054,26702556:22749088,451360,127400
x1,79:9411054,26702556
g1,78:9629454,26702556
x1,78:9957054,26702556
g1,78:10175454,26702556
x1,78:12759854,26702556
g1,78:12978254,26702556
x1,78:14179454,26702556
g1,78:14397854,26702556
x1,78:16363454,26702556
x1,78:17473654,26702556
g1,78:17692054,26702556
x1,78:18476474,26702556
g1,78:18694874,26702556
x1,78:22118294,26702556
g1,78:22336694,26702556
x1,78:22627894,26702556
x1,78:24105734,26702556
k1,79:31614142,26702556:7508408
g1,79:31614142,26702556
)
(1,81:8865054,28265005:22749088,976821,937531
x1,81:9285804,28265005
(1,81:9285804,28475814:1927030,436543,238108
x1,81:9548556,28475814
[1,81:9548556,28606885:334511,489697,0
(1,81:9579125,28344743:303942,227555,0
x1,81:9850299,28344743
)
(1,81:9548556,28606885:332044,141084,0
x1,81:9847832,28606885
)
]
x1,81:10668288,28475814
[1,81:10668288,28650207:511778,610936,63715
(1,81:10698857,28317800:481209,278529,0
x1,81:10970031,28317800
(1,81:10970031,28221316:177267,182045,0
x1,81:11114530,28221316
)
)
(1,81:10668288,28650207:308682,227555,63715
x1,81:10927363,28650207
)
]
)
x1,81:12168570,28265005
k1,81:12350610,28265005:182040
x1,81:12860336,28265005
k1,81:13042376,28265005:182040
[1,81:13042376,28265005:946633,688132,927973
(1,81:13042376,28265005:946633,688132,360452
(1,81:13042376,27642409:946633,65536,983048
x1,81:13989009,27642409
)
)
(1,81:13042376,29038241:946633,303558,89201
k1,81:13223473,29038241:181097
x1,81:13781404,29038241
k1,81:13989009,29038241:181096
)
]
k1,81:14098233,28265005:109224
[1,81:14098233,28265005:946633,688132,937531
(1,81:14098233,28265005:946633,688132,360452
(1,81:14098233,27642409:946633,65536,983048
x1,81:15044866,27642409
)
)
(1,81:14098233,29047799:946633,313116,89201
k1,81:14157738,29047799:59505
x1,81:14808094,29047799
(1,81:14808094,28916728:177267,182045,0
x1,81:14952593,28916728
)
k1,81:15044866,29047799:59505
)
]
k1,81:15154090,28265005:109224
x1,81:15601555,28265005
[1,81:15601555,28427021:538930,646056,89201
(1,81:15673006,27994412:301284,213447,0
x1,81:15941522,27994412
)
(1,81:15601555,28427021:538930,318577,89201
x1,81:15898722,28427021
x1,81:16107717,28427021
)
]
x1,81:16587950,28265005
(1,81:16587950,28363308:558894,303558,0
x1,81:17114076,28363308
)
x1,81:17594309,28265005
(1,81:17594309,28363308:596882,318577,89201
x1,81:17891476,28363308
x1,81:18131914,28363308
)
x1,81:18638656,28265005
[1,81:18638656,28427021:616846,646056,89201
(1,81:18710107,27994412:301284,213447,0
x1,81:18978623,27994412
)
(1,81:18638656,28427021:616846,303558,89201
x1,81:19196225,28427021
)
]
x1,81:19723902,28265005
[1,81:19723902,28427021:870557,812428,0
(1,81:19770778,27994412:823681,379819,0
x1,81:20384424,27994412
(1,81:20384424,27796638:177267,182045,0
x1,81:20528923,27796638
)
)
(1,81:19723902,28427021:465542,303558,0
x1,81:20156676,28427021
)
]
x1,81:21062859,28265005
[1,81:21062859,28427021:870557,812428,89201
(1,81:21109735,27994412:823681,379819,0
x1,81:21723381,27994412
(1,81:21723381,27796638:177267,182045,0
x1,81:21867880,27796638
)
)
(1,81:21062859,28427021:700761,313116,89201
x1,81:21279722,28427021
x1,81:21553585,28427021
(1,81:21553585,28295950:177267,182045,0
x1,81:21698084,28295950
)
)
]
k1,81:22042640,28265005:109224
(1,81:22042640,28265005:1001247,282168,127431
x1,81:23043887,28265005
)
k1,81:23153111,28265005:109224
(1,80:23153111,28265005:391396,753669,425990
$1,80:23153111,28265005
(1,80:23153111,28265005:391396,753669,425990
(1,80:23153111,27537549:391396,26213,1153446
x1,80:23544507,27537549
)
v1,80:23544507,28265005:0,753664,0
h1,80:23544507,28265005:0,0,0
)
$1,80:23544507,28265005
)
k1,81:23544507,28265005:0
x1,81:24054233,28265005
k1,81:24054233,28265005:0
x1,81:24981267,28265005
(1,81:25004780,28265005:1736831,891184,632593
(1,81:25004780,28265005:1736831,891184,632593
h1,81:25004780,28265005:78643,0,0
[1,81:25083423,28265005:1579545,891184,632593
(1,81:25083423,27821649:1579545,447828,0
k1,81:25650191,27821649:566768
x1,81:26096201,27821649
k1,81:26662968,27821649:566767
)
(1,81:25083423,28820961:1579545,628051,76636
x1,81:25529433,28820961
[1,81:25529433,28897597:1133535,704687,0
(1,81:25529433,28506026:1133535,313116,89201
x1,81:25931716,28506026
x1,81:26452933,28506026
(1,81:26452933,28374955:177267,182045,0
x1,81:26597432,28374955
)
)
(1,81:25529433,28897597:773016,197518,0
x1,81:26269681,28897597
)
]
)
]
h1,81:26662968,28265005:78643,0,0
)
)
(1,80:26741611,28265005:391396,753669,425990
$1,80:26741611,28265005
(1,80:26741611,28265005:391396,753669,425990
(1,80:26741611,27537549:391396,26213,1153446
x1,80:27133007,27537549
)
v1,80:27133007,28265005:0,753664,0
h1,80:27133007,28265005:0,0,0
)
$1,80:27133007,28265005
)
k1,81:27242231,28265005:109224
(1,81:27242231,28265005:1001247,282168,127431
x1,81:28243478,28265005
)
k1,81:28352702,28265005:109224
(1,80:28352702,28265005:391396,753669,425990
$1,80:28352702,28265005
(1,80:28352702,28265005:391396,753669,425990
(1,80:28352702,27537549:391396,26213,1153446
x1,80:28744098,27537549
)
v1,80:28744098,28265005:0,753664,0
h1,80:28744098,28265005:0,0,0
)
$1,80:28744098,28265005
)
k1,81:28744098,28265005:0
x1,81:29253824,28265005
k1,81:29253824,28265005:0
(1,81:29253824,28265005:2540560,976821,753652
(1,81:29253824,28265005:2540560,976821,753652
h1,81:29253824,28265005:78643,0,0
[1,81:29332467,28265005:2383274,976821,753652
(1,81:29332467,27821649:2383274,533465,0
k1,81:30154098,27821649:821631
x1,81:30600108,27821649
(1,81:30600108,27583824:294003,295640,0
x1,81:30861343,27583824
)
k1,81:31715741,27821649:821630
)
(1,81:29332467,28820961:2383274,628051,197695
x1,81:30033340,28820961
[1,81:30033340,29018656:1133535,825746,0
(1,81:30033340,28506026:1133535,313116,89201
x1,81:30435623,28506026
x1,81:30956840,28506026
(1,81:30956840,28374955:177267,182045,0
x1,81:31101339,28374955
)
)
(1,81:30033340,29018656:832485,318577,0
x1,81:30833057,29018656
)
]
x1,81:31421738,28820961
(1,81:31421738,28631635:294003,295640,0
x1,81:31682973,28631635
)
)
]
h1,81:31715741,28265005:78643,0,0
)
)
(1,80:31794384,28265005:391396,753669,425990
$1,80:31794384,28265005
(1,80:31794384,28265005:391396,753669,425990
(1,80:31794384,27537549:391396,26213,1153446
x1,80:32185780,27537549
)
v1,80:32185780,28265005:0,753664,0
h1,80:32185780,28265005:0,0,0
)
$1,80:32185780,28265005
)
x1,80:32367825,28265005
)
(1,81:30776942,29759472:837200,491400,163800
(1,81:30776942,29759472:837200,491400,163800
x1,81:31614142,29759472
)
)
(1,84:8865054,30545904:22749088,451360,127400
h1,83:8865054,30545904:983040,0,0
x1,83:11524314,30545904
g1,83:11742714,30545904
x1,83:12652714,30545904
g1,83:12871114,30545904
x1,83:14916794,30545904
x1,83:16864194,30545904
g1,83:17082594,30545904
x1,83:20220274,30545904
g1,83:20438674,30545904
x1,83:21494274,30545904
g1,83:21712674,30545904
x1,83:24480894,30545904
g1,83:24699294,30545904
x1,83:26741334,30545904
g1,83:26959734,30545904
x1,83:27835154,30545904
g1,83:28053554,30545904
x1,83:28599554,30545904
x1,83:29420374,30545904
x1,83:31112974,30545904
k1,84:31614142,30545904:501168
g1,84:31614142,30545904
)
(1,85:8865054,31332336:22749088,0,0
h1,85:8865054,31332336:983040,0,0
k1,85:31614142,31332336:21766048
g1,85:31614142,31332336
)
(1,89:15440719,32435782:16173423,1037910,738633
(1,89:15440719,32435782:9597758,1037910,738633
x1,89:15886729,32435782
[1,89:15886729,32597798:1133535,812428,0
(1,89:15886729,32165189:1133535,379819,89201
x1,89:16289012,32165189
x1,89:16810229,32165189
(1,89:16810229,31967415:177267,182045,0
x1,89:16954728,31967415
)
)
(1,89:15886729,32597798:773016,197518,0
x1,89:16626977,32597798
)
]
g1,89:17202304,32435782
x1,89:17712030,32435782
g1,89:17894070,32435782
(1,89:17894070,32435782:1293473,725524,738633
(1,89:17894070,32435782:1293473,725524,738633
h1,89:17894070,32435782:78643,0,0
[1,89:17972713,32435782:1136187,725524,738633
(1,89:17972713,31992426:1136187,282168,0
k1,89:18342264,31992426:369551
x1,89:18715837,31992426
k1,89:19108900,31992426:369550
)
(1,89:17972713,32902537:1136187,538850,271877
x1,89:18380644,32902537
[1,89:18380644,33085213:728256,721526,89201
(1,89:18404157,32676803:704743,313116,0
x1,89:18898865,32676803
(1,89:18898865,32545732:177267,182045,0
x1,89:19043364,32545732
)
)
(1,89:18380644,33085213:461560,303558,89201
x1,89:18782927,33085213
)
]
)
]
h1,89:19108900,32435782:78643,0,0
)
)
x1,89:19369588,32435782
g1,87:19551628,32435782
g1,87:19733668,32435782
g1,87:19915708,32435782
g1,89:20024932,32435782
x1,89:20470942,32435782
[1,89:20470942,32633477:1133535,892449,0
(1,89:20470942,32120847:1133535,379819,89201
x1,89:20873225,32120847
x1,89:21394442,32120847
(1,89:21394442,31923073:177267,182045,0
x1,89:21538941,31923073
)
)
(1,89:20470942,32633477:832485,318577,0
x1,89:21270659,32633477
)
]
g1,89:21786517,32435782
x1,89:22296243,32435782
g1,89:22478283,32435782
(1,89:22478283,32435782:2378149,1037910,738633
(1,89:22478283,32435782:2378149,1037910,738633
h1,89:22478283,32435782:78643,0,0
[1,89:22556926,32435782:2220863,1037910,738633
(1,89:22556926,31992426:2220863,594554,98303
k1,89:22714391,31992426:157465
x1,89:23042072,31992426
(1,89:23042072,31992426:873816,594554,87018
(1,89:23042072,31450298:546135,26213,629146
x1,89:23588207,31450298
)
[1,89:23588207,31992426:327681,594554,0
(1,89:23588207,31992426:327681,422343,0
x1,89:23915888,31992426
)
]
)
x1,89:24290369,31992426
(1,89:24290369,32090729:329956,197518,0
x1,89:24587557,32090729
)
k1,89:24777789,31992426:157464
)
(1,89:22556926,32902537:2220863,538850,271877
x1,89:22874594,32902537
[1,89:22874594,33085213:303635,605928,0
(1,89:22898107,32676803:280122,197518,0
x1,89:23145461,32676803
)
(1,89:22874594,33085213:218188,303558,0
x1,89:23060014,33085213
)
]
g1,89:23323861,32902537
x1,89:23833587,32902537
g1,89:23979219,32902537
x1,89:24296887,32902537
[1,89:24296887,33085213:480902,721526,89201
(1,89:24320400,32676803:457389,313116,0
x1,89:24567754,32676803
(1,89:24567754,32545732:177267,182045,0
x1,89:24712253,32545732
)
)
(1,89:24296887,33085213:276140,303558,89201
x1,89:24513750,33085213
)
]
)
]
h1,89:24777789,32435782:78643,0,0
)
)
x1,89:25038477,32435782
)
(1,89:30776942,32435782:837200,491400,163800
(1,89:30776942,32435782:837200,491400,163800
x1,89:31614142,32435782
)
)
)
(1,92:8865054,34282458:22749088,806891,315196
h1,91:8865054,34282458:983040,0,0
x1,91:10976494,34282458
k1,91:11128428,34282458:151934
x1,91:14266108,34282458
k1,91:14418043,34282458:151935
x1,91:17553903,34282458
k1,91:17705837,34282458:151934
$1,91:17705837,34282458
x1,91:18113768,34282458
[1,91:18113768,34453043:623785,605928,89201
(1,91:18137281,34044633:600272,197518,0
x1,91:18688325,34044633
)
(1,91:18113768,34453043:461560,303558,89201
x1,91:18516051,34453043
)
]
$1,91:18737553,34282458
k1,91:18889488,34282458:151935
x1,91:19764908,34282458
k1,91:19916842,34282458:151934
x1,91:20772242,34282458
x1,91:21409242,34282458
k1,91:21561177,34282458:151935
x1,91:21925177,34282458
x1,91:22252777,34282458
k1,91:22404711,34282458:151934
$1,91:22404711,34282458
x1,91:22812642,34282458
[1,91:22812642,34453043:623785,605928,89201
(1,91:22836155,34044633:600272,197518,0
x1,91:23387199,34044633
)
(1,91:22812642,34453043:461560,303558,89201
x1,91:23214925,34453043
)
]
x1,91:24021018,34282458
(1,91:24021018,34380761:294003,295640,0
x1,91:24282253,34380761
)
x1,91:24569884,34282458
k1,91:24751924,34282458:182040
x1,91:25261650,34282458
k1,91:25443690,34282458:182040
(1,91:25443690,34282458:1479828,806891,315196
(1,91:25443690,34282458:1479828,806891,315196
h1,91:25443690,34282458:78643,0,0
[1,91:25522333,34282458:1322542,806891,315196
(1,91:25522333,33884512:1322542,408945,194786
x1,91:26425202,33884512
[1,91:26425202,34015583:419673,540016,63715
(1,91:26425202,33686738:255776,211171,0
x1,91:26648210,33686738
)
(1,91:26425202,34015583:419673,218388,63715
x1,91:26792782,34015583
)
]
)
(1,91:25522333,34508452:1322542,295640,89201
k1,91:25790018,34508452:267685
x1,91:26321415,34508452
(1,91:26321415,34573988:255776,211171,0
x1,91:26544423,34573988
)
k1,91:26844875,34508452:267684
)
]
h1,91:26844875,34282458:78643,0,0
)
)
k1,91:26936190,34282458:12672
x1,91:27445916,34282458
k1,91:27458588,34282458:12672
x1,91:28108337,34282458
(1,91:28108337,34380761:218188,303558,0
x1,91:28293757,34380761
)
x1,91:28633725,34282458
k1,91:28646396,34282458:12671
x1,91:29156122,34282458
k1,91:29168794,34282458:12672
x1,91:29563680,34282458
(1,91:29563680,34380761:276140,303558,89201
x1,91:29780543,34380761
)
x1,91:30214301,34282458
x1,91:30989773,34282458
(1,91:30989773,34380761:442369,318577,0
x1,91:31399374,34380761
)
$1,91:31432142,34282458
x1,91:31614142,34282458
k1,92:31614142,34282458:0
k1,92:31614142,34282458:0
)
(1,94:8865054,35154590:22749088,491400,163800
h1,93:8865054,35154590:983040,0,0
x1,93:10976494,35154590
k1,93:11248355,35154590:271861
x1,93:11834395,35154590
x1,93:12489595,35154590
x1,93:12999195,35154590
x1,93:14386035,35154590
k1,93:14657896,35154590:271861
x1,93:15970116,35154590
x1,93:16297716,35154590
x1,93:17025716,35154590
x1,93:17207716,35154590
x1,93:18194156,35154590
k1,93:18466017,35154590:271861
x1,93:19048417,35154590
h1,93:19048417,35154590:0,0,0
x1,93:19303217,35154590
k1,93:19575078,35154590:271861
x1,93:20557878,35154590
x1,93:21105698,35154590
x1,93:21615298,35154590
x1,93:22379698,35154590
k1,93:22651558,35154590:271860
x1,93:23561558,35154590
k1,93:23833419,35154590:271861
x1,93:24470419,35154590
x1,93:25640679,35154590
x1,93:27031159,35154590
k1,93:27303020,35154590:271861
x1,93:27776220,35154590
x1,93:28049220,35154590
k1,93:28321081,35154590:271861
x1,93:29012681,35154590
x1,93:30796281,35154590
k1,93:31068142,35154590:271861
x1,93:31614142,35154590
k1,93:31614142,35154590:0
)
(1,94:8865054,35941022:22749088,491400,163800
x1,94:9884254,35941022
k1,93:10144100,35941022:259846
x1,93:11199700,35941022
k1,93:11459546,35941022:259846
x1,93:12078346,35941022
x1,93:13425146,35941022
x1,93:13661746,35941022
k1,93:13921593,35941022:259847
x1,93:14706013,35941022
k1,93:14965859,35941022:259846
x1,93:15602859,35941022
x1,93:15966859,35941022
x1,93:16312659,35941022
x1,93:16967859,35941022
x1,93:17331859,35941022
x1,93:18260059,35941022
k1,93:18519905,35941022:259846
x1,93:20121505,35941022
x1,93:20995105,35941022
k1,93:21254951,35941022:259846
x1,93:21782751,35941022
k1,93:22042597,35941022:259846
x1,93:23061797,35941022
x1,93:24446817,35941022
k1,93:24706663,35941022:259846
x1,93:25292703,35941022
x1,93:25947903,35941022
x1,93:26457503,35941022
x1,93:27844343,35941022
k1,93:28104190,35941022:259847
x1,93:28686590,35941022
k1,93:28946436,35941022:259846
x1,93:30331456,35941022
k1,93:30591302,35941022:259846
x1,93:31395742,35941022
x1,93:31614142,35941022
k1,94:31614142,35941022:0
)
(1,94:8865054,36727454:22749088,491400,163800
x1,94:10393854,36727454
k1,93:10573048,36727454:179194
x1,93:11592248,36727454
k1,93:11771442,36727454:179194
x1,93:12353842,36727454
k1,93:12533036,36727454:179194
x1,93:13006236,36727454
x1,93:13315636,36727454
x1,93:13643236,36727454
x1,93:13916236,36727454
k1,93:14095430,36727454:179194
x1,93:15078230,36727454
x1,93:15405830,36727454
x1,93:16192070,36727454
k1,93:16371264,36727454:179194
x1,93:17284904,36727454
x1,93:17612504,36727454
x1,93:18196724,36727454
x1,93:19507124,36727454
k1,93:19686318,36727454:179194
x1,93:20436158,36727454
x1,93:21309758,36727454
k1,93:21488952,36727454:179194
x1,93:22071352,36727454
h1,93:22071352,36727454:0,0,0
x1,93:22508152,36727454
k1,93:22687346,36727454:179194
x1,93:23160546,36727454
x1,93:23433546,36727454
k1,93:23612740,36727454:179194
x1,93:24304340,36727454
x1,93:25432740,36727454
k1,93:25611934,36727454:179194
x1,93:26521934,36727454
k1,93:26701128,36727454:179194
x1,93:27410928,36727454
x1,93:27920528,36727454
x1,93:28375528,36727454
x1,93:29249128,36727454
k1,93:29428322,36727454:179194
x1,93:30119922,36727454
x1,93:31068142,36727454
x1,93:31395742,36727454
x1,93:31614142,36727454
k1,94:31614142,36727454:0
)
(1,94:8865054,37513886:22749088,451360,127431
x1,94:9047054,37513886
x1,94:10466654,37513886
g1,93:10685054,37513886
x1,93:11322054,37513886
x1,93:12492314,37513886
x1,93:13882794,37513886
g1,93:14101194,37513886
x1,93:14885614,37513886
g1,93:15104014,37513886
x1,93:16014014,37513886
g1,93:16232414,37513886
x1,93:16851214,37513886
x1,93:17763034,37513886
x1,93:19000634,37513886
g1,93:19219034,37513886
x1,93:21261074,37513886
g1,93:21479474,37513886
x1,93:22334874,37513886
x1,93:22971874,37513886
g1,93:23190274,37513886
x1,93:24391474,37513886
g1,93:24609874,37513886
$1,93:24609874,37513886
x1,93:24939602,37513886
g1,93:25121642,37513886
x1,93:25777003,37513886
g1,93:25959043,37513886
x1,93:26534458,37513886
(1,93:26534458,37612189:218188,303558,0
x1,93:26719878,37612189
)
g1,93:26934686,37513886
x1,93:27590047,37513886
g1,93:27772087,37513886
x1,93:28166973,37513886
(1,93:28166973,37612189:218188,303558,0
x1,93:28352393,37612189
)
x1,93:28882257,37513886
$1,93:28915138,37513886
x1,93:29097138,37513886
k1,94:31614142,37513886:2517004
g1,94:31614142,37513886
)
(1,95:8865054,38300318:22749088,0,0
h1,95:8865054,38300318:983040,0,0
k1,95:31614142,38300318:21766048
g1,95:31614142,38300318
)
(1,99:12479332,39403764:19134810,1037910,721422
(1,99:12479332,39403764:15520533,1037910,721422
x1,99:12925342,39403764
[1,99:12925342,39601459:956268,816188,0
(1,99:12925342,39088829:956268,303558,89201
x1,99:13327625,39088829
x1,99:13848842,39088829
)
(1,99:12925342,39601459:832485,318577,0
x1,99:13725059,39601459
)
]
g1,99:14063650,39403764
x1,99:14573376,39403764
g1,99:14755416,39403764
(1,99:14755416,39403764:2686951,1037910,721422
(1,99:14755416,39403764:2686951,1037910,721422
h1,99:14755416,39403764:78643,0,0
[1,99:14834059,39403764:2529665,1037910,721422
(1,99:14834059,38960408:2529665,594554,127431
x1,99:15161740,38960408
(1,99:15161740,38960408:873816,594554,87018
(1,99:15161740,38418280:546135,26213,629146
x1,99:15707875,38418280
)
[1,99:15707875,38960408:327681,594554,0
(1,99:15707875,38960408:327681,422343,0
x1,99:16035556,38960408
)
]
)
x1,99:16410037,38960408
(1,99:16410037,39058711:329956,197518,0
x1,99:16707225,39058711
)
x1,99:17069721,38960408
(1,99:17069721,38722583:294003,295640,0
x1,99:17330956,38722583
)
)
(1,99:14834059,39853308:2529665,521374,271877
k1,99:15307337,39853308:473278
x1,99:16428887,39853308
[1,99:16428887,40035984:461560,704050,89201
(1,99:16428887,39627574:294003,295640,0
x1,99:16690122,39627574
)
(1,99:16428887,40035984:461560,303558,89201
x1,99:16831170,40035984
)
]
k1,99:17363724,39853308:473277
)
]
h1,99:17363724,39403764:78643,0,0
)
)
x1,99:17624412,39403764
g1,96:17806452,39403764
g1,96:17988492,39403764
g1,96:18170532,39403764
g1,99:18279756,39403764
x1,99:18725766,39403764
[1,99:18725766,39601459:1215529,781601,0
(1,99:18725766,39123416:1215529,303558,54614
x1,99:19908527,39123416
)
(1,99:18725766,39601459:832485,318577,0
x1,99:19525483,39601459
)
]
g1,99:20123335,39403764
x1,99:20633061,39403764
g1,99:20815101,39403764
(1,99:20815101,39403764:2169755,976821,632221
(1,99:20815101,39403764:2169755,976821,632221
h1,99:20815101,39403764:78643,0,0
[1,99:20893744,39403764:2012469,976821,632221
(1,99:20893744,38960408:2012469,533465,127431
k1,99:21235895,38960408:342151
x1,99:21610376,38960408
(1,99:21610376,39058711:329956,197518,0
x1,99:21907564,39058711
)
x1,99:22270060,38960408
(1,99:22270060,38722583:294003,295640,0
x1,99:22531295,38722583
)
k1,99:22906213,38960408:342150
)
(1,99:20893744,39853308:2012469,521374,182676
x1,99:21288630,39853308
(1,99:21288630,39951611:218188,303558,0
x1,99:21474050,39951611
)
x1,99:22003914,39853308
x1,99:22612210,39853308
[1,99:22612210,40035984:294003,704050,0
(1,99:22612210,39627574:294003,295640,0
x1,99:22873445,39627574
)
(1,99:22612210,40035984:218188,303558,0
x1,99:22797630,40035984
)
]
)
]
h1,99:22906213,39403764:78643,0,0
)
)
x1,99:23166901,39403764
g1,97:23348941,39403764
g1,97:23530981,39403764
g1,97:23713021,39403764
g1,99:23822245,39403764
x1,99:24268255,39403764
[1,99:24268255,39601459:1273481,816188,0
(1,99:24268255,39088829:1273481,303558,89201
x1,99:24670538,39088829
x1,99:25508968,39088829
)
(1,99:24268255,39601459:832485,318577,0
x1,99:25067972,39601459
)
]
g1,99:25723776,39403764
x1,99:26233502,39403764
g1,99:26415542,39403764
x1,99:26861552,39403764
[1,99:26861552,39601459:956268,816188,0
(1,99:26861552,39088829:956268,303558,89201
x1,99:27263835,39088829
x1,99:27785052,39088829
)
(1,99:26861552,39601459:832485,318577,0
x1,99:27661269,39601459
)
]
x1,99:27999865,39403764
)
(1,99:30776942,39403764:837200,491400,163800
(1,99:30776942,39403764:837200,491400,163800
x1,99:31614142,39403764
)
)
)
(1,101:8865054,41044830:22749088,618493,197695
x1,101:10195474,41044830
k1,100:10416370,41044830:220896
x1,100:11326370,41044830
k1,100:11547265,41044830:220895
x1,100:12166065,41044830
x1,100:13077885,41044830
x1,100:14315485,41044830
k1,100:14536381,41044830:220896
x1,100:16578421,41044830
k1,100:16799316,41044830:220895
$1,100:16799316,41044830
x1,100:17245326,41044830
[1,100:17245326,41242525:956268,816188,0
(1,100:17245326,40729895:956268,303558,89201
x1,100:17647609,40729895
x1,100:18168826,40729895
)
(1,100:17245326,41242525:832485,318577,0
x1,100:18045043,41242525
)
]
$1,100:18201594,41044830
k1,100:18422490,41044830:220896
x1,100:19478090,41044830
k1,100:19698985,41044830:220895
$1,100:19698985,41044830
x1,100:20144995,41044830
[1,100:20144995,41242525:1215529,781601,0
(1,100:20144995,40764482:1215529,303558,54614
x1,100:21327756,40764482
)
(1,100:20144995,41242525:832485,318577,0
x1,100:20944712,41242525
)
]
$1,100:21360524,41044830
k1,100:21581420,41044830:220896
x1,100:22236620,41044830
x1,100:23588880,41044830
x1,100:23898280,41044830
k1,100:24119175,41044830:220895
x1,100:25720775,41044830
x1,100:26594375,41044830
k1,100:26815271,41044830:220896
x1,100:27343071,41044830
k1,100:27563966,41044830:220895
x1,100:28150006,41044830
x1,100:28805206,41044830
x1,100:29314806,41044830
x1,100:30701646,41044830
k1,100:30922542,41044830:220896
x1,100:31614142,41044830
k1,100:31614142,41044830:0
)
(1,101:8865054,41831262:22749088,588001,473606
x1,101:9210854,41831262
x1,101:9793254,41831262
x1,101:11067254,41831262
k1,100:11300109,41831262:232855
x1,100:13342149,41831262
k1,100:13575005,41831262:232856
$1,100:13575005,41831262
x1,100:14021015,41831262
[1,100:14021015,41993278:956268,703399,0
(1,100:14021015,41593437:956268,303558,89201
x1,100:14423298,41593437
x1,100:14944515,41593437
)
(1,100:14021015,41993278:773016,197518,0
x1,100:14761263,41993278
)
]
k1,100:15183420,41831262:206137
x1,100:15693146,41831262
k1,100:15899284,41831262:206138
(1,100:15899284,41831262:1479828,588001,473606
(1,100:15899284,41831262:1479828,588001,473606
h1,100:15899284,41831262:78643,0,0
[1,100:15977927,41831262:1322542,588001,473606
(1,100:15977927,41538901:1322542,295640,89201
k1,100:16212036,41538901:234109
x1,100:16779738,41538901
x1,100:17066360,41538901
k1,100:17300469,41538901:234109
)
(1,100:15977927,42075926:1322542,369185,228941
x1,100:16880796,42075926
[1,100:16880796,42241152:419673,534411,63715
(1,100:16880796,41917912:255776,211171,0
x1,100:17103804,41917912
)
(1,100:16880796,42241152:419673,218388,63715
x1,100:17248376,42241152
)
]
)
]
h1,100:17300469,41831262:78643,0,0
)
)
$1,100:17379112,41831262
k1,100:17611967,41831262:232855
x1,100:18667567,41831262
k1,100:18900423,41831262:232856
x1,100:20101623,41831262
x1,100:21484823,41831262
k1,100:21717678,41831262:232855
x1,100:23759718,41831262
k1,100:23992573,41831262:232855
$1,100:23992573,41831262
x1,100:24438583,41831262
[1,100:24438583,41993278:1215529,703399,0
(1,100:24438583,41593437:1215529,303558,54614
x1,100:25621344,41593437
)
(1,100:24438583,41993278:773016,197518,0
x1,100:25178831,41993278
)
]
k1,100:25860250,41831262:206138
x1,100:26369976,41831262
k1,100:26576114,41831262:206138
(1,100:26576114,41831262:1467293,455554,315196
(1,100:26576114,41831262:1467293,455554,315196
h1,100:26576114,41831262:78643,0,0
[1,100:26654757,41831262:1310007,455554,315196
(1,100:26654757,41573226:1310007,197518,0
k1,100:27148297,41573226:493540
x1,100:27454764,41573226
k1,100:27964764,41573226:493540
)
(1,100:26654757,42057256:1310007,313481,89201
x1,100:26973414,42057256
(1,100:26973414,42122792:207608,218388,0
x1,100:27148254,42122792
)
x1,100:27577005,42057256
(1,100:27577005,42126797:387759,227555,0
x1,100:27931996,42126797
)
)
]
h1,100:27964764,41831262:78643,0,0
)
)
$1,100:28043407,41831262
k1,100:28276262,41831262:232855
x1,100:29151682,41831262
x1,100:29699502,41831262
x1,100:30321942,41831262
x1,100:31395742,41831262
x1,100:31614142,41831262
k1,101:31614142,41831262:0
)
(1,101:8865054,42821764:22749088,451360,127400
x1,101:10266454,42821764
x1,101:10393854,42821764
k1,100:10670767,42821764:276913
x1,100:12035767,42821764
k1,100:12312680,42821764:276913
x1,100:13513880,42821764
k1,100:13790792,42821764:276912
x1,100:14518792,42821764
x1,100:15228592,42821764
x1,100:15501592,42821764
k1,100:15778505,42821764:276913
x1,100:16688505,42821764
k1,100:16965418,42821764:276913
x1,100:17584218,42821764
x1,100:18496038,42821764
x1,100:19733638,42821764
k1,100:20010551,42821764:276913
x1,100:22052591,42821764
k1,100:22329504,42821764:276913
x1,100:22857304,42821764
k1,100:23134216,42821764:276912
x1,100:23480016,42821764
x1,100:24062416,42821764
x1,100:25336416,42821764
k1,100:25613329,42821764:276913
x1,100:26632529,42821764
x1,100:28017549,42821764
k1,100:28294462,42821764:276913
x1,100:28880502,42821764
x1,100:29535702,42821764
x1,100:30045302,42821764
x1,100:31614142,42821764
k1,100:31614142,42821764:0
)
(1,101:8865054,43608196:22749088,583906,197695
x1,101:9775054,43608196
g1,100:9993454,43608196
x1,100:10612254,43608196
x1,100:11524074,43608196
x1,100:12761674,43608196
g1,100:12980074,43608196
x1,100:14763674,43608196
g1,100:14982074,43608196
$1,100:14982074,43608196
x1,100:15428084,43608196
[1,100:15428084,43805891:1215529,781601,0
(1,100:15428084,43327848:1215529,303558,54614
x1,100:16610845,43327848
)
(1,100:15428084,43805891:832485,318577,0
x1,100:16227801,43805891
)
]
$1,100:16643613,43608196
g1,100:16862013,43608196
x1,100:17302453,43608196
g1,100:17520853,43608196
x1,100:18469073,43608196
x1,100:18833073,43608196
x1,100:19435493,43608196
x1,100:21073493,43608196
g1,100:21291893,43608196
x1,100:21874293,43608196
g1,100:22092693,43608196
x1,100:23002693,43608196
g1,100:23221093,43608196
x1,100:24240293,43608196
x1,100:24549693,43608196
g1,100:24768093,43608196
x1,100:25295893,43608196
g1,100:25514293,43608196
x1,100:26533493,43608196
x1,100:27918513,43608196
g1,100:28136913,43608196
x1,100:29010513,43608196
x1,100:29847713,43608196
x1,100:30211713,43608196
x1,100:31540313,43608196
k1,101:31614142,43608196:73829
g1,101:31614142,43608196
)
]
(1,103:8865054,45574276:22749088,0,0
h1,103:8865054,45574276:22749088,0,0
)
]
]
!50286
}2
!10
{3
[1,136:4736286,45574276:26877856,40837990,0
(1,136:4736286,4736286:0,0,0
[1,136:0,4736286:0,0,0
(1,136:0,0:0,0,0
g1,136:0,0
)
]
)
[1,136:8865054,45574276:22749088,39789414,0
[1,136:8865054,6571294:22749088,786432,0
(1,136:8865054,6571294:22749088,406224,114660
(1,136:8865054,6571294:22749088,406224,114660
k1,136:13956475,6571294:5091421
(1,40:13956475,6571294:15483450,406224,114660
x1,40:14579278,6571294
x1,40:14831802,6571294
x1,40:15134831,6571294
x1,40:15387583,6571294
g1,40:15589603,6571294
x1,40:16498692,6571294
x1,40:16801721,6571294
x1,40:17290162,6571294
g1,40:17492182,6571294
x1,40:19884570,6571294
x1,40:20103423,6571294
g1,40:20305443,6571294
x1,40:20793658,6571294
g1,40:20995678,6571294
x1,40:23219489,6571294
g1,40:23421509,6571294
x1,40:23909724,6571294
g1,40:24111744,6571294
x1,40:26335555,6571294
g1,40:26537575,6571294
x1,40:29439925,6571294
)
g1,136:31614142,6571294
(1,136:31614142,6571294:0,379288,0
k1,136:31311112,6571294:-303030
x1,136:31614142,6571294
)
)
)
]
[1,136:8865054,43608196:22749088,35988326,0
[1,118:8865054,20728855:22749088,13108985,0
[1,118:8865054,20728855:22749088,13108985,0
(1,117:8865054,18517043:22749088,10897173,0
k1,117:8991410,18517043:126356
h1,113:8991410,18517043:0,0,0
(1,113:8991410,18517043:11147178,10897173,0
(1,113:8991410,18517043:11146849,10897200,0
(1,113:8991410,18517043:11146849,10897200,0
(1,113:8991410,18517043:0,10897200,0
(1,113:8991410,18517043:0,41347783,0
(1,113:8991410,18517043:42295040,41347783,0
)
k1,113:8991410,18517043:-42295040
)
)
g1,113:20138259,18517043
)
)
)
g1,113:20340608,18517043
(1,115:20340608,18517043:11147178,10897173,0
(1,115:20340608,18517043:11146849,10897200,0
(1,115:20340608,18517043:11146849,10897200,0
(1,115:20340608,18517043:0,10897200,0
(1,115:20340608,18517043:0,41347783,0
(1,115:20340608,18517043:42295040,41347783,0
)
k1,115:20340608,18517043:-42295040
)
)
g1,115:31487457,18517043
)
)
)
g1,117:31487786,18517043
k1,117:31614142,18517043:126356
)
(1,117:8865054,19893299:22749088,407043,114660
h1,117:8865054,19893299:0,0,0
x1,117:10040136,19893299
x1,117:10699161,19893299
k1,117:10855053,19893299:155892
k1,117:10855053,19893299:0
x1,117:11722010,19893299
x1,117:12025039,19893299
x1,117:12884987,19893299
k1,117:13040879,19893299:155892
x1,117:14455018,19893299
x1,117:16465114,19893299
k1,117:16621006,19893299:155892
x1,117:17109221,19893299
k1,117:17265113,19893299:155892
x1,117:19727980,19893299
k1,117:19883872,19893299:155892
x1,117:21769391,19893299
k1,117:21925283,19893299:155892
x1,117:23155602,19893299
k1,117:23311495,19893299:155893
x1,117:24153472,19893299
k1,117:24309364,19893299:155892
x1,117:26502097,19893299
k1,117:26657989,19893299:155892
x1,117:27533636,19893299
x1,117:28259131,19893299
k1,117:28415023,19893299:155892
x1,117:29140292,19893299
k1,117:29296184,19893299:155892
x1,117:30138161,19893299
k1,117:30294053,19893299:155892
x1,117:31614142,19893299
k1,117:31614142,19893299:0
)
(1,117:8865054,20614195:22749088,406224,114660
x1,117:9353269,20614195
g1,117:9555289,20614195
x1,117:11779100,20614195
g1,117:11981120,20614195
x1,117:14883470,20614195
g1,117:15085490,20614195
x1,117:15590540,20614195
g1,117:15792560,20614195
x1,117:16112425,20614195
x1,117:17829593,20614195
g1,117:18031613,20614195
x1,117:19008043,20614195
g1,117:19210063,20614195
x1,117:19715113,20614195
g1,117:19917133,20614195
x1,117:20220163,20614195
g1,117:20422183,20614195
x1,117:22812979,20614195
g1,117:23014999,20614195
x1,117:24294687,20614195
k1,117:31614142,20614195:7319455
g1,117:31614142,20614195
)
]
]
(1,103:8865054,23489089:22749088,451360,127400
h1,102:8865054,23489089:983040,0,0
x1,102:10448694,23489089
x1,102:12980314,23489089
k1,102:13154009,23489089:173695
x1,102:14428009,23489089
k1,102:14601704,23489089:173695
x1,102:14929304,23489089
k1,102:15102998,23489089:173694
x1,102:16304198,23489089
x1,102:17687398,23489089
k1,102:17861093,23489089:173695
x1,102:19062293,23489089
k1,102:19235988,23489089:173695
x1,102:20109588,23489089
x1,102:20437188,23489089
k1,102:20610883,23489089:173695
x1,102:21484483,23489089
x1,102:21866683,23489089
x1,102:22594683,23489089
k1,102:22768378,23489089:173695
x1,102:23459978,23489089
x1,102:23787578,23489089
x1,102:24717598,23489089
k1,102:24891292,23489089:173694
x1,102:26056092,23489089
x1,102:26420092,23489089
x1,102:26765892,23489089
x1,102:27206332,23489089
x1,102:28334732,23489089
k1,102:28508427,23489089:173695
x1,102:29036227,23489089
k1,102:29209922,23489089:173695
x1,102:30229122,23489089
x1,102:31614142,23489089
k1,102:31614142,23489089:0
)
(1,103:8865054,24275521:22749088,451360,127400
x1,103:9702254,24275521
x1,103:10029854,24275521
x1,103:10976254,24275521
x1,103:11849854,24275521
k1,102:12049030,24275521:199176
x1,102:13379450,24275521
k1,102:13578626,24275521:199176
x1,102:14164666,24275521
x1,102:15003686,24275521
x1,102:15731686,24275521
x1,102:16317726,24275521
x1,102:16499726,24275521
x1,102:17300526,24275521
k1,102:17499702,24275521:199176
x1,102:17827302,24275521
x1,102:18191302,24275521
x1,102:19705542,24275521
k1,102:19904718,24275521:199176
x1,102:21069518,24275521
x1,102:22421778,24275521
k1,102:22620954,24275521:199176
x1,102:23405374,24275521
k1,102:23604550,24275521:199176
x1,102:24241550,24275521
x1,102:25115150,24275521
x1,102:25952350,24275521
k1,102:26151526,24275521:199176
x1,102:27607526,24275521
x1,102:29483946,24275521
k1,102:29683122,24275521:199176
x1,102:30702322,24275521
x1,102:31395742,24275521
x1,102:31614142,24275521
k1,103:31614142,24275521:0
)
(1,103:8865054,25061953:22749088,451360,127400
x1,103:9815094,25061953
k1,102:10023887,25061953:208793
x1,102:11117707,25061953
x1,102:11299707,25061953
x1,102:12246107,25061953
x1,102:13119707,25061953
k1,102:13328501,25061953:208794
x1,102:14658921,25061953
k1,102:14867714,25061953:208793
x1,102:15777714,25061953
k1,102:15986508,25061953:208794
x1,102:17629058,25061953
x1,102:18357058,25061953
k1,102:18565851,25061953:208793
x1,102:19148251,25061953
x1,102:19512251,25061953
x1,102:20478671,25061953
k1,102:20687465,25061953:208794
x1,102:21815865,25061953
k1,102:22024658,25061953:208793
x1,102:22716258,25061953
x1,102:23043858,25061953
x1,102:23973878,25061953
k1,102:24182672,25061953:208794
x1,102:25347472,25061953
x1,102:25711472,25061953
x1,102:26057272,25061953
x1,102:26497712,25061953
x1,102:27626112,25061953
k1,102:27834905,25061953:208793
x1,102:28417305,25061953
k1,102:28626099,25061953:208794
x1,102:29430539,25061953
x1,102:30959339,25061953
k1,102:31168132,25061953:208793
$1,102:31168132,25061953
x1,102:31614142,25061953
$1,102:31614142,25061953
k1,103:31614142,25061953:0
)
(1,103:8865054,25848385:22749088,451360,127400
x1,103:9305494,25848385
g1,102:9523894,25848385
x1,102:10379294,25848385
x1,102:11016294,25848385
g1,102:11234694,25848385
x1,102:11598694,25848385
x1,102:11926294,25848385
k1,103:31614142,25848385:19687848
g1,103:31614142,25848385
)
(1,105:16794083,27946680:14820059,985662,735357
(1,105:16794083,27946680:6891031,985662,735357
x1,105:17089754,27946680
(1,105:17089754,28044983:373474,197518,0
x1,105:17430460,28044983
)
x1,105:18418964,27946680
g1,105:18601004,27946680
x1,105:19110730,27946680
g1,105:19292770,27946680
(1,105:19292770,27946680:4392344,985662,735357
(1,105:19292770,27946680:4392344,985662,735357
h1,105:19292770,27946680:78643,0,0
[1,105:19371413,27946680:4235058,985662,735357
(1,105:19371413,27494483:4235058,533465,196611
k1,105:19531784,27494483:160371
(1,105:19531784,27002959:691771,0,655368
x1,105:20223555,27002959
)
(1,105:20223555,27691094:373474,197518,0
x1,105:20564261,27691094
)
g1,105:20706253,27494483
x1,105:21001924,27494483
[1,105:21001924,27656499:373474,695481,0
(1,105:21020129,27256658:294003,295640,0
x1,105:21281364,27256658
)
(1,105:21001924,27656499:373474,197518,0
x1,105:21342630,27656499
)
]
x1,105:21796148,27494483
(1,105:21796148,27592786:694216,318577,89201
x1,105:22434021,27592786
)
x1,105:23446100,27494483
k1,105:23606471,27494483:160371
)
(1,105:19371413,28396224:4235058,491524,285812
(1,105:19371413,27904700:691771,0,655368
x1,105:20063184,27904700
)
(1,105:20063184,28592835:694216,318577,89201
x1,105:20701057,28592835
)
g1,105:20866624,28396224
x1,105:21162295,28396224
[1,105:21162295,28558240:373474,646982,0
(1,105:21180500,28206898:294003,295640,0
x1,105:21441735,28206898
)
(1,105:21162295,28558240:373474,197518,0
x1,105:21503001,28558240
)
]
x1,105:21956519,28396224
(1,105:21956519,28494527:694216,318577,89201
x1,105:22594392,28494527
)
x1,105:23606471,28396224
)
]
h1,105:23606471,27946680:78643,0,0
)
)
)
(1,105:30776942,27946680:837200,491400,163800
(1,105:30776942,27946680:837200,491400,163800
x1,105:31614142,27946680
)
)
)
(1,107:8865054,30593951:22749088,533465,394303
x1,107:10541274,30593951
k1,106:10715446,30593951:174172
$1,106:10715446,30593951
x1,106:11011117,30593951
[1,106:11011117,30779555:353510,719069,89201
(1,106:11029322,30356126:294003,295640,0
x1,106:11290557,30356126
)
(1,106:11011117,30779555:353510,318577,89201
x1,106:11308284,30779555
)
]
$1,106:11364627,30593951
k1,106:11538800,30593951:174173
x1,106:12414220,30593951
k1,106:12588392,30593951:174172
x1,106:13498392,30593951
k1,106:13672565,30593951:174173
x1,106:14364165,30593951
x1,106:14691765,30593951
x1,106:15621785,30593951
k1,106:15795958,30593951:174173
x1,106:17403018,30593951
k1,106:17577190,30593951:174172
x1,106:18159590,30593951
k1,106:18333762,30593951:174172
x1,106:20122822,30593951
k1,106:20296995,30593951:174173
x1,106:21352595,30593951
k1,106:21526768,30593951:174173
$1,106:21526768,30593951
x1,106:21947518,30593951
(1,106:21947518,30692254:694216,318577,89201
x1,106:22585391,30692254
)
k1,106:22823774,30593951:182040
x1,106:23333500,30593951
k1,106:23515540,30593951:182040
x1,106:23936290,30593951
(1,106:23936290,30750146:1833655,381929,238108
x1,106:24199042,30750146
[1,106:24199042,30881217:376457,486057,0
(1,106:24229611,30619075:345888,223915,0
x1,106:24542731,30619075
)
(1,106:24199042,30881217:332044,141084,0
x1,106:24498318,30881217
)
]
x1,106:25360720,30750146
[1,106:25360720,30924539:376457,556322,63715
(1,106:25391289,30592132:345888,223915,0
x1,106:25704409,30592132
)
(1,106:25360720,30924539:308682,227555,63715
x1,106:25619795,30924539
)
]
)
$1,106:25769945,30593951
k1,106:25944117,30593951:174172
x1,106:26819537,30593951
k1,106:26993710,30593951:174173
x1,106:27903710,30593951
k1,106:28077882,30593951:174172
x1,106:31614142,30593951
k1,106:31614142,30593951:0
)
(1,107:8865054,31505150:22749088,451360,0
x1,107:9392854,31505150
g1,106:9611254,31505150
x1,106:10302854,31505150
x1,106:10630454,31505150
x1,106:11560474,31505150
g1,106:11778874,31505150
x1,106:15098554,31505150
k1,107:31614142,31505150:16515588
g1,107:31614142,31505150
)
(1,110:8865054,32598148:22749088,451360,127400
h1,108:8865054,32598148:983040,0,0
x1,108:10976494,32598148
k1,108:11232970,32598148:256476
x1,108:11853590,32598148
x1,108:12181190,32598148
x1,108:13218590,32598148
x1,108:14346990,32598148
k1,108:14603466,32598148:256476
x1,108:15731866,32598148
x1,108:16077666,32598148
x1,108:16405266,32598148
x1,108:17755706,32598148
k1,108:18012182,32598148:256476
x1,108:18539982,32598148
k1,108:18796458,32598148:256476
x1,108:20252458,32598148
x1,108:22128878,32598148
k1,108:22385354,32598148:256476
x1,108:23404554,32598148
x1,108:24097974,32598148
x1,108:25048014,32598148
k1,108:25304490,32598148:256476
x1,108:25744930,32598148
k1,108:26001406,32598148:256476
x1,108:27826866,32598148
x1,108:28591266,32598148
k1,108:28847742,32598148:256476
x1,108:29575742,32598148
x1,108:30613142,32598148
x1,108:31614142,32598148
k1,108:31614142,32598148:0
)
(1,110:8865054,33384580:22749088,533465,0
x1,110:9483854,33384580
x1,108:10088094,33384580
k1,108:10237106,33384580:149012
x1,108:11147106,33384580
k1,108:11296119,33384580:149013
x1,108:12024119,33384580
x1,108:12970519,33384580
k1,108:13119531,33384580:149012
x1,108:13811131,33384580
x1,108:14138731,33384580
x1,108:15068751,33384580
k1,108:15217764,33384580:149013
x1,108:15801984,33384580
x1,108:16824824,33384580
k1,108:16973836,33384580:149012
$1,108:16973836,33384580
x1,108:17269507,33384580
(1,108:17287712,33146755:294003,295640,0
x1,108:17548947,33146755
)
$1,108:17581715,33384580
k1,108:17730727,33384580:149012
x1,108:18606147,33384580
k1,108:18755160,33384580:149013
x1,108:19483160,33384580
x1,108:20322180,33384580
x1,108:21632580,33384580
k1,108:21781592,33384580:149012
x1,108:22454992,33384580
x1,108:22691592,33384580
k1,108:22840605,33384580:149013
x1,108:23823405,33384580
x1,108:25175665,33384580
k1,108:25324677,33384580:149012
x1,108:25870677,33384580
x1,108:26800697,33384580
x1,108:27455897,33384580
x1,108:27692497,33384580
k1,108:27841510,33384580:149013
x1,108:28569510,33384580
x1,108:29515910,33384580
k1,108:29664922,33384580:149012
x1,108:30356522,33384580
x1,108:30684122,33384580
x1,108:31614142,33384580
k1,108:31614142,33384580:0
)
(1,110:8865054,34171012:22749088,451360,127400
x1,110:9449274,34171012
x1,110:10654114,34171012
k1,108:10829213,34171012:175099
x1,108:11415253,34171012
k1,108:11590352,34171012:175099
x1,108:12063552,34171012
x1,108:12700552,34171012
k1,108:12875651,34171012:175099
x1,108:13461691,34171012
k1,108:13636790,34171012:175099
x1,108:14182790,34171012
x1,108:15112810,34171012
x1,108:15768010,34171012
x1,108:16004610,34171012
k1,108:16179709,34171012:175099
x1,108:16525509,34171012
x1,108:16998709,34171012
x1,108:17912349,34171012
k1,108:18087448,34171012:175099
x1,108:18615248,34171012
k1,108:18790347,34171012:175099
x1,108:19809547,34171012
x1,108:21194567,34171012
k1,108:21369666,34171012:175099
x1,108:22570866,34171012
x1,108:23954066,34171012
k1,108:24129165,34171012:175099
x1,108:25002765,34171012
x1,108:26203965,34171012
x1,108:26699005,34171012
k1,108:26874104,34171012:175099
x1,108:28204524,34171012
k1,108:28379623,34171012:175099
x1,108:29289623,34171012
k1,108:29464722,34171012:175099
x1,108:29646722,34171012
x1,108:30010722,34171012
x1,108:30795142,34171012
x1,108:31140942,34171012
x1,108:31614142,34171012
k1,108:31614142,34171012:0
)
(1,110:8865054,34957444:22749088,533465,163840
x1,110:10139369,34957444
k1,108:10248593,34957444:109224
x1,108:11340863,34957444
k1,108:11518193,34957444:177330
x1,108:12027919,34957444
k1,108:12205249,34957444:177330
x1,108:12860611,34957444
(1,108:12860611,34719619:964839,295640,54614
x1,108:13792682,34719619
)
x1,108:14220336,34957444
(1,108:14220336,35055747:451084,313481,0
x1,108:14616319,35055747
)
$1,108:14671420,34957444
x1,108:14853420,34957444
k1,108:15119356,34957444:265936
x1,108:15719956,34957444
k1,108:15985892,34957444:265936
x1,108:17432792,34957444
h1,108:17432792,34957444:0,0,0
k1,108:17698728,34957444:265936
x1,108:18171928,34957444
x1,108:18444928,34957444
k1,108:18710865,34957444:265937
x1,108:19660905,34957444
x1,108:20115905,34957444
k1,108:20381841,34957444:265936
x1,108:21291841,34957444
k1,108:21557777,34957444:265936
x1,108:21921777,34957444
x1,108:22526017,34957444
x1,108:22966457,34957444
x1,108:23803657,34957444
k1,108:24069593,34957444:265936
x1,108:24761193,34957444
x1,108:25088793,34957444
x1,108:26018813,34957444
k1,108:26284750,34957444:265937
x1,108:26868970,34957444
x1,108:27891810,34957444
k1,108:28157746,34957444:265936
x1,108:28685546,34957444
k1,108:28951482,34957444:265936
x1,108:29970682,34957444
x1,108:30664102,34957444
x1,108:31614142,34957444
k1,108:31614142,34957444:0
)
(1,110:8865054,35743876:22749088,451360,127400
x1,110:10177274,35743876
x1,110:10504874,35743876
x1,110:11414874,35743876
x1,110:12288474,35743876
k1,108:12519283,35743876:230809
x1,108:13849703,35743876
k1,108:14080512,35743876:230809
x1,108:14990512,35743876
k1,108:15221321,35743876:230809
x1,108:16863871,35743876
x1,108:17591871,35743876
k1,108:17822680,35743876:230809
x1,108:18405080,35743876
x1,108:18769080,35743876
x1,108:19553500,35743876
k1,108:19784309,35743876:230809
x1,108:20366709,35743876
k1,108:20597517,35743876:230808
x1,108:20925117,35743876
k1,108:21155926,35743876:230809
x1,108:21958546,35743876
x1,108:22764806,35743876
x1,108:23967826,35743876
k1,108:24198635,35743876:230809
x1,108:25217835,35743876
x1,108:26602855,35743876
k1,108:26833664,35743876:230809
x1,108:27852864,35743876
x1,108:29094104,35743876
x1,108:29403504,35743876
k1,108:29634313,35743876:230809
x1,108:30418733,35743876
k1,108:30649542,35743876:230809
x1,108:31195542,35743876
x1,108:31614142,35743876
k1,110:31614142,35743876:0
)
(1,110:8865054,36530308:22749088,451360,127431
x1,110:9613074,36530308
x1,110:10268274,36530308
x1,110:10504874,36530308
k1,108:10740362,36530308:235488
x1,108:11086162,36530308
x1,108:11559362,36530308
x1,108:12473002,36530308
k1,108:12708491,36530308:235489
x1,108:13236291,36530308
k1,108:13471779,36530308:235488
x1,108:14490979,36530308
x1,108:15875999,36530308
k1,108:16111487,36530308:235488
x1,108:17312687,36530308
x1,108:18695887,36530308
k1,108:18931376,36530308:235489
x1,108:19804976,36530308
x1,108:21006176,36530308
x1,108:21501216,36530308
k1,108:21736704,36530308:235488
$1,108:21736704,36530308
x1,108:22131590,36530308
(1,108:22131590,36628611:294003,295640,0
x1,108:22392825,36628611
)
x1,108:22607638,36530308
k1,108:22716862,36530308:109224
x1,108:23111748,36530308
(1,108:23111748,36628611:294003,295640,0
x1,108:23372983,36628611
)
x1,108:23587796,36530308
k1,108:23697020,36530308:109224
x1,108:24091906,36530308
(1,108:24091906,36628611:294003,295640,0
x1,108:24353141,36628611
)
$1,108:24385909,36530308
k1,108:24621397,36530308:235488
x1,108:25676997,36530308
k1,108:25912485,36530308:235488
x1,108:26640485,36530308
x1,108:27586885,36530308
k1,108:27822374,36530308:235489
x1,108:28513974,36530308
x1,108:28841574,36530308
x1,108:29771594,36530308
k1,108:30007082,36530308:235488
x1,108:30591302,36530308
x1,108:31614142,36530308
k1,108:31614142,36530308:0
)
(1,110:8865054,37316740:22749088,533465,127431
x1,110:9160725,37316740
(1,108:9178930,37078915:294003,295640,0
x1,108:9440165,37078915
)
$1,108:9472933,37316740
k1,108:9755035,37316740:282102
x1,108:10341075,37316740
x1,108:11509515,37316740
x1,108:12383115,37316740
k1,108:12665218,37316740:282103
x1,108:14121218,37316740
x1,108:14849218,37316740
k1,108:15131320,37316740:282102
x1,108:16332520,37316740
x1,108:17715720,37316740
k1,108:17997823,37316740:282103
x1,108:19199023,37316740
k1,108:19481125,37316740:282102
x1,108:21852585,37316740
k1,108:22134688,37316740:282103
$1,108:22134688,37316740
x1,108:22631784,37316740
k1,108:22952899,37316740:288234
x1,108:23462625,37316740
k1,108:23750859,37316740:288234
x1,108:24473426,37316740
$1,108:24473426,37316740
x1,108:24987576,37316740
k1,108:25269615,37316740:282039
x1,108:26325215,37316740
k1,108:26607317,37316740:282102
x1,108:27772117,37316740
x1,108:29011537,37316740
k1,108:29293640,37316740:282103
x1,108:30749640,37316740
k1,108:31031742,37316740:282102
x1,108:31614142,37316740
k1,108:31614142,37316740:0
)
(1,110:8865054,38103172:22749088,451360,127400
x1,110:10106294,38103172
k1,108:10317945,38103172:211651
x1,108:11229765,38103172
x1,108:12976965,38103172
k1,108:13188615,38103172:211650
x1,108:13552615,38103172
x1,108:13880215,38103172
k1,108:14091866,38103172:211651
x1,108:15001866,38103172
k1,108:15213517,38103172:211651
x1,108:15559317,38103172
x1,108:16141717,38103172
x1,108:17415717,38103172
k1,108:17627367,38103172:211650
x1,108:18646567,38103172
x1,108:20031587,38103172
k1,108:20243238,38103172:211651
x1,108:20829278,38103172
x1,108:21484478,38103172
x1,108:21994078,38103172
x1,108:23380918,38103172
k1,108:23592569,38103172:211651
x1,108:24943009,38103172
k1,108:25154659,38103172:211650
x1,108:26485079,38103172
k1,108:26696730,38103172:211651
x1,108:27169930,38103172
x1,108:27442930,38103172
k1,108:27654581,38103172:211651
x1,108:28873981,38103172
x1,108:29146981,38103172
k1,108:29358631,38103172:211650
x1,108:29686231,38103172
k1,108:29897882,38103172:211651
x1,108:30445702,38103172
x1,108:30955302,38103172
x1,108:31395742,38103172
x1,108:31614142,38103172
k1,110:31614142,38103172:0
)
(1,110:8865054,38889604:22749088,533465,251217
x1,110:9593054,38889604
k1,108:9818890,38889604:225836
x1,108:10404930,38889604
x1,108:11937370,38889604
x1,108:13065770,38889604
k1,108:13291606,38889604:225836
x1,108:14492806,38889604
k1,108:14718642,38889604:225836
x1,108:16176462,38889604
k1,108:16402298,38889604:225836
x1,108:16842738,38889604
k1,108:17068574,38889604:225836
x1,108:17760174,38889604
k1,108:17986010,38889604:225836
x1,108:18932410,38889604
k1,108:19158245,38889604:225835
x1,108:20177445,38889604
x1,108:20870865,38889604
x1,108:21820905,38889604
k1,108:22046741,38889604:225836
x1,108:22629141,38889604
k1,108:22854977,38889604:225836
x1,108:24826037,38889604
k1,108:25051873,38889604:225836
x1,108:25889073,38889604
k1,108:26114909,38889604:225836
$1,108:26114909,38889604
x1,108:26410580,38889604
(1,108:26428785,38651779:294003,295640,0
x1,108:26690020,38651779
)
k1,108:26917224,38889604:194436
x1,108:27426950,38889604
k1,108:27621386,38889604:194436
x1,108:28171920,38889604
[1,108:28171920,39051620:312208,695481,0
(1,108:28190125,38651779:294003,295640,0
x1,108:28451360,38651779
)
(1,108:28171920,39051620:281419,197518,0
x1,108:28420571,39051620
)
]
x1,108:28666173,38889604
k1,108:28775397,38889604:109224
x1,108:29071068,38889604
[1,108:29071068,39051620:351425,695481,89201
(1,108:29089273,38651779:294003,295640,0
x1,108:29350508,38651779
)
(1,108:29071068,39051620:351425,197518,89201
x1,108:29389725,39051620
)
]
x1,108:29604538,38889604
k1,108:29713762,38889604:109224
x1,108:30296306,38889604
$1,108:30296306,38889604
x1,108:30478306,38889604
k1,108:30704142,38889604:225836
x1,108:31377542,38889604
x1,108:31614142,38889604
k1,108:31614142,38889604:0
)
(1,110:8865054,39676036:22749088,451360,127400
x1,110:9957054,39676036
k1,108:10157800,39676036:200746
x1,108:11359000,39676036
k1,108:11559746,39676036:200746
x1,108:12578946,39676036
x1,108:13963966,39676036
k1,108:14164711,39676036:200745
x1,108:14346711,39676036
x1,108:14710711,39676036
x1,108:15495131,39676036
x1,108:16113931,39676036
x1,108:17242331,39676036
k1,108:17443077,39676036:200746
x1,108:18717077,39676036
k1,108:18917823,39676036:200746
x1,108:19827823,39676036
k1,108:20028569,39676036:200746
x1,108:21671119,39676036
x1,108:22399119,39676036
k1,108:22599865,39676036:200746
x1,108:23801065,39676036
x1,108:25184265,39676036
k1,108:25385010,39676036:200745
x1,108:26586210,39676036
k1,108:26786956,39676036:200746
x1,108:27660556,39676036
x1,108:27988156,39676036
k1,108:28188902,39676036:200746
x1,108:28956942,39676036
x1,108:29502942,39676036
x1,108:29866942,39676036
x1,108:30849742,39676036
x1,108:31614142,39676036
k1,108:31614142,39676036:0
)
(1,110:8865054,40462468:22749088,451360,127400
x1,110:9738654,40462468
x1,110:10120854,40462468
x1,110:10848854,40462468
k1,108:11105226,40462468:256372
x1,108:12015226,40462468
k1,108:12271597,40462468:256371
x1,108:12963197,40462468
x1,108:14115257,40462468
x1,108:14752257,40462468
k1,108:15008629,40462468:256372
x1,108:15700229,40462468
x1,108:16027829,40462468
x1,108:16957849,40462468
k1,108:17214221,40462468:256372
x1,108:17798441,40462468
x1,108:18562841,40462468
k1,108:18819212,40462468:256371
x1,108:19201412,40462468
k1,108:19457784,40462468:256372
x1,108:20476984,40462468
x1,108:21862004,40462468
k1,108:22118375,40462468:256371
x1,108:23319575,40462468
x1,108:24702775,40462468
k1,108:24959147,40462468:256372
x1,108:25832747,40462468
x1,108:27033947,40462468
x1,108:27528987,40462468
k1,108:27785359,40462468:256372
x1,108:28660779,40462468
k1,108:28917150,40462468:256371
x1,108:29863550,40462468
k1,108:30119922,40462468:256372
x1,108:30629522,40462468
x1,108:31084522,40462468
x1,108:31614142,40462468
k1,108:31614142,40462468:0
)
(1,110:8865054,41248900:22749088,533465,163840
x1,110:10175454,41248900
k1,108:10472729,41248900:297275
$1,108:10472729,41248900
x1,108:10994470,41248900
x1,108:11922900,41248900
(1,108:11922900,41011075:964839,295640,54614
x1,108:12854971,41011075
)
x1,108:13282625,41248900
(1,108:13282625,41347203:451084,313481,0
x1,108:13678608,41347203
)
x1,108:13988572,41248900
$1,108:13988572,41248900
x1,108:14170572,41248900
k1,108:14467847,41248900:297275
x1,108:15669047,41248900
k1,108:15966322,41248900:297275
x1,108:16406762,41248900
k1,108:16704037,41248900:297275
x1,108:17288257,41248900
x1,108:18200077,41248900
k1,108:18497352,41248900:297275
x1,108:19025152,41248900
k1,108:19322427,41248900:297275
x1,108:20523627,41248900
x1,108:21069627,41248900
x1,108:22343627,41248900
k1,108:22640902,41248900:297275
x1,108:24282542,41248900
k1,108:24579817,41248900:297275
x1,108:25890217,41248900
k1,108:26187492,41248900:297275
x1,108:27097492,41248900
k1,108:27394767,41248900:297275
x1,108:28781607,41248900
k1,108:29078882,41248900:297275
x1,108:30394742,41248900
x1,108:31377542,41248900
x1,108:31614142,41248900
k1,108:31614142,41248900:0
)
(1,110:8865054,42035332:22749088,451360,127400
x1,110:9776874,42035332
x1,110:10688694,42035332
x1,110:10925294,42035332
k1,108:11180397,42035332:255103
x1,108:12272397,42035332
x1,108:13056817,42035332
x1,108:13420817,42035332
x1,108:15040617,42035332
k1,108:15295720,42035332:255103
x1,108:16132920,42035332
x1,108:16919160,42035332
k1,108:17174263,42035332:255103
x1,108:17647463,42035332
x1,108:17920463,42035332
k1,108:18175566,42035332:255103
x1,108:19158366,42035332
x1,108:20650766,42035332
k1,108:20905870,42035332:255104
x1,108:22107070,42035332
k1,108:22362173,42035332:255103
x1,108:23381373,42035332
x1,108:24766393,42035332
k1,108:25021496,42035332:255103
x1,108:26222696,42035332
x1,108:27605896,42035332
k1,108:27860999,42035332:255103
x1,108:28734599,42035332
x1,108:29935799,42035332
x1,108:30430839,42035332
k1,108:30685942,42035332:255103
x1,108:31049942,42035332
x1,108:31395742,42035332
x1,108:31614142,42035332
k1,110:31614142,42035332:0
)
(1,110:8865054,42821764:22749088,451360,127400
x1,110:9411054,42821764
x1,110:9775054,42821764
x1,110:11231054,42821764
k1,108:11507148,42821764:276094
x1,108:12489948,42821764
k1,108:12766042,42821764:276094
x1,108:13130042,42821764
x1,108:13439442,42821764
k1,108:13715535,42821764:276093
x1,108:15027755,42821764
x1,108:15701155,42821764
k1,108:15977249,42821764:276094
x1,108:16341249,42821764
x1,108:16668849,42821764
k1,108:16944943,42821764:276094
x1,108:17964143,42821764
x1,108:19349163,42821764
k1,108:19625257,42821764:276094
x1,108:20644457,42821764
x1,108:21885697,42821764
x1,108:22635537,42821764
k1,108:22911631,42821764:276094
x1,108:23825271,42821764
x1,108:24171071,42821764
k1,108:24447164,42821764:276093
x1,108:25033204,42821764
k1,108:25309298,42821764:276094
x1,108:26128298,42821764
x1,108:27329498,42821764
x1,108:27820898,42821764
k1,108:28096992,42821764:276094
x1,108:29416492,42821764
x1,108:30108092,42821764
x1,108:31614142,42821764
k1,108:31614142,42821764:0
)
(1,110:8865054,43608196:22749088,451360,0
x1,110:9920654,43608196
g1,108:10139054,43608196
x1,108:13014654,43608196
k1,110:31614142,43608196:18599488
g1,110:31614142,43608196
)
]
(1,136:8865054,45574276:22749088,0,0
h1,136:8865054,45574276:22749088,0,0
)
]
]
!27046
}3
!10
{4
[1,194:4736286,45574276:26877856,40837990,0
(1,194:4736286,4736286:0,0,0
[1,194:0,4736286:0,0,0
(1,194:0,0:0,0,0
g1,194:0,0
)
]
)
[1,194:8865054,45574276:22749088,39789414,0
[1,194:8865054,6571294:22749088,786432,0
(1,194:8865054,6571294:22749088,406224,114660
(1,194:8865054,6571294:22749088,406224,114660
(1,194:8865054,6571294:0,379288,0
x1,194:9168084,6571294
k1,194:8865054,6571294:-303030
)
g1,194:11039271,6571294
(1,40:11039271,6571294:4032070,406224,114660
x1,40:11662074,6571294
g1,40:11864094,6571294
x1,40:12276506,6571294
x1,40:12899400,6571294
x1,40:13219265,6571294
x1,40:13522294,6571294
g1,40:13724314,6571294
x1,40:14229591,6571294
g1,40:14431611,6571294
x1,40:15071341,6571294
)
k1,194:31614142,6571294:16542801
)
)
]
[1,194:8865054,43608196:22749088,35988326,0
(1,129:8865054,8275230:22749088,542724,0
(1,129:8865054,8275230:0,0,0
g1,129:8865054,8275230
)
x1,129:13004093,8275230
k1,129:31614141,8275230:18610048
g1,129:31614141,8275230
)
(1,135:9664114,9782558:21950028,442260,147420
(1,130:9664114,9782558:0,379288,0
g1,130:9664114,9782558
g1,130:9192734,9782558
g1,130:8865054,9782558
(1,130:8865054,9782558:471380,379288,0
g1,130:8865054,9782558
x1,130:9336434,9782558
)
g1,130:9664114,9782558
)
x1,130:10244876,9782558
k1,131:10408547,9782558:163671
x1,131:12043042,9782558
k1,131:12206714,9782558:163672
x1,131:12686284,9782558
k1,131:12867623,9782558:181339
x1,131:13517361,9782558
k1,131:13681033,9782558:163672
x1,131:16096534,9782558
k1,131:16260167,9782558:163633
x1,131:17977336,9782558
x1,131:20217754,9782558
k1,131:20381425,9782558:163671
x1,131:21130537,9782558
k1,133:20381425,9782558:-16836
x1,133:21840972,9782558
k1,133:22004643,9782558:163671
x1,133:23208528,9782558
k1,133:23372200,9782558:163672
x1,133:24660257,9782558
k1,133:24823928,9782558:163671
x1,133:25870610,9782558
k1,133:26034281,9782558:163671
x1,133:27717779,9782558
k1,133:27881451,9782558:163672
x1,133:29463941,9782558
k1,133:29627612,9782558:163671
x1,133:31614142,9782558
k1,135:31614142,9782558:0
k1,135:31614142,9782558:0
)
(1,140:9664114,10503454:21950028,442260,147420
(1,136:9664114,10503454:0,379288,0
g1,136:9664114,10503454
g1,136:9192734,10503454
g1,136:8865054,10503454
(1,136:8865054,10503454:471380,379288,0
g1,136:8865054,10503454
x1,136:9336434,10503454
)
g1,136:9664114,10503454
)
x1,136:10270173,10503454
g1,137:10472193,10503454
x1,137:11789509,10503454
x1,137:12345062,10503454
g1,137:12547082,10503454
x1,137:13169885,10503454
g1,137:13371905,10503454
x1,137:16385597,10503454
g1,137:16587617,10503454
g1,139:16789637,10503454
x1,139:17993522,10503454
g1,139:18195542,10503454
x1,139:19054036,10503454
x1,139:19575921,10503454
g1,139:19777941,10503454
x1,139:20527053,10503454
x1,139:21237488,10503454
g1,139:21439508,10503454
x1,139:22305646,10503454
g1,139:22507666,10503454
x1,139:23416756,10503454
g1,139:23618776,10503454
x1,139:25302274,10503454
k1,140:31614142,10503454:6311868
g1,140:31614142,10503454
)
(1,147:9664114,11224350:21950028,442260,147420
(1,142:9664114,11224350:0,379288,0
g1,142:9664114,11224350
g1,142:9192734,11224350
g1,142:8865054,11224350
(1,142:8865054,11224350:471380,379288,0
g1,142:8865054,11224350
x1,142:9336434,11224350
)
g1,142:9664114,11224350
)
x1,142:10270173,11224350
g1,143:10472193,11224350
x1,143:11789509,11224350
x1,143:12176712,11224350
g1,143:12378732,11224350
x1,143:13355162,11224350
g1,143:13557182,11224350
x1,143:14163241,11224350
g1,143:14365261,11224350
x1,143:14988064,11224350
g1,143:15190084,11224350
x1,143:15627793,11224350
x1,143:17097623,11224350
g1,143:17299643,11224350
x1,143:18048755,11224350
k1,145:17299643,11224350:-16836
x1,145:18759190,11224350
g1,145:18961210,11224350
x1,145:20165095,11224350
g1,145:20367115,11224350
x1,145:20830032,11224350
g1,145:21032052,11224350
x1,145:22078734,11224350
g1,145:22280754,11224350
x1,145:23964252,11224350
g1,145:24166272,11224350
x1,145:25445732,11224350
g1,145:25647752,11224350
x1,145:27634282,11224350
k1,147:31614142,11224350:3979860
g1,147:31614142,11224350
)
(1,152:9664114,11945246:21950028,442260,147420
(1,148:9664114,11945246:0,379288,0
g1,148:9664114,11945246
g1,148:9192734,11945246
g1,148:8865054,11945246
(1,148:8865054,11945246:471380,379288,0
g1,148:8865054,11945246
x1,148:9336434,11945246
)
g1,148:9664114,11945246
)
x1,148:10278546,11945246
g1,149:10480566,11945246
x1,149:11448760,11945246
x1,149:11920139,11945246
g1,149:12122159,11945246
x1,149:13207788,11945246
g1,151:13409808,11945246
x1,151:14840782,11945246
g1,151:15042802,11945246
x1,151:15995298,11945246
x1,151:16449842,11945246
g1,151:16651862,11945246
x1,151:18047438,11945246
g1,151:18249458,11945246
x1,151:19932956,11945246
g1,151:20134976,11945246
x1,151:21414436,11945246
g1,151:21616456,11945246
x1,151:22424536,11945246
x1,151:23198946,11945246
k1,152:31614142,11945246:8415196
g1,152:31614142,11945246
)
(1,159:9664114,12666142:21950028,442260,147420
(1,154:9664114,12666142:0,379288,0
g1,154:9664114,12666142
g1,154:9192734,12666142
g1,154:8865054,12666142
(1,154:8865054,12666142:471380,379288,0
g1,154:8865054,12666142
x1,154:9336434,12666142
)
g1,154:9664114,12666142
)
x1,154:10270173,12666142
g1,155:10472193,12666142
x1,155:11789509,12666142
x1,155:12345062,12666142
g1,155:12547082,12666142
x1,155:12942659,12666142
k1,157:12547082,12666142:-50506
x1,157:14373633,12666142
g1,157:14575653,12666142
x1,157:15324765,12666142
x1,157:16035200,12666142
g1,157:16237220,12666142
x1,157:17525277,12666142
g1,157:17727297,12666142
x1,157:18425085,12666142
g1,157:18627105,12666142
x1,157:20478953,12666142
g1,157:20680973,12666142
x1,157:21792083,12666142
x1,157:22869523,12666142
k1,159:31614142,12666142:8744619
g1,159:31614142,12666142
)
(1,166:9664114,13387038:21950028,442260,147420
(1,161:9664114,13387038:0,379288,0
g1,161:9664114,13387038
g1,161:9192734,13387038
g1,161:8865054,13387038
(1,161:8865054,13387038:471380,379288,0
g1,161:8865054,13387038
x1,161:9336434,13387038
)
g1,161:9664114,13387038
)
x1,161:10143866,13387038
g1,162:10345886,13387038
x1,162:10951945,13387038
g1,162:11153965,13387038
x1,162:11566377,13387038
x1,162:13974236,13387038
g1,162:14176256,13387038
x1,162:15152686,13387038
g1,162:15354706,13387038
x1,162:15977509,13387038
g1,162:16179529,13387038
x1,162:18940697,13387038
g1,162:19142717,13387038
x1,162:20733396,13387038
k1,164:19142717,13387038:0
g1,164:20935416,13387038
x1,164:21633204,13387038
g1,164:21835224,13387038
x1,164:23687072,13387038
g1,164:23889092,13387038
x1,164:24966532,13387038
k1,166:31614142,13387038:6647610
g1,166:31614142,13387038
)
(1,173:9664114,14107934:21950028,442260,147420
(1,168:9664114,14107934:0,379288,0
g1,168:9664114,14107934
g1,168:9192734,14107934
g1,168:8865054,14107934
(1,168:8865054,14107934:471380,379288,0
g1,168:8865054,14107934
x1,168:9336434,14107934
)
g1,168:9664114,14107934
)
x1,168:10143866,14107934
g1,169:10345886,14107934
x1,169:12404849,14107934
g1,169:12606869,14107934
x1,169:13583299,14107934
g1,169:13785319,14107934
x1,169:14408122,14107934
g1,169:14610142,14107934
x1,169:15232945,14107934
g1,169:15434965,14107934
x1,169:17321849,14107934
x1,169:17793228,14107934
g1,169:17995248,14107934
x1,169:19149764,14107934
g1,171:19351784,14107934
x1,171:20100896,14107934
x1,171:20811331,14107934
g1,171:21013351,14107934
x1,171:21493103,14107934
g1,171:21695123,14107934
x1,171:22132832,14107934
g1,171:22334852,14107934
x1,171:23032640,14107934
g1,171:23234660,14107934
x1,171:24918158,14107934
g1,171:25120178,14107934
x1,171:26399638,14107934
g1,171:26601658,14107934
x1,171:27679098,14107934
k1,173:31614142,14107934:3935044
g1,173:31614142,14107934
)
(1,180:9664114,14828830:21950028,442260,147420
(1,175:9664114,14828830:0,379288,0
g1,175:9664114,14828830
g1,175:9192734,14828830
g1,175:8865054,14828830
(1,175:8865054,14828830:471380,379288,0
g1,175:8865054,14828830
x1,175:9336434,14828830
)
g1,175:9664114,14828830
)
x1,175:10244876,14828830
g1,176:10446896,14828830
x1,176:12972282,14828830
x1,176:13443661,14828830
g1,176:13645681,14828830
x1,176:14125433,14828830
g1,176:14327453,14828830
x1,176:14798741,14828830
x1,176:15758335,14828830
g1,176:15960355,14828830
x1,176:16936785,14828830
g1,176:17138805,14828830
x1,176:17862619,14828830
g1,176:18064639,14828830
x1,176:20296822,14828830
g1,176:20498842,14828830
x1,176:22114818,14828830
k1,178:20498842,14828830:0
g1,178:22316838,14828830
x1,178:23014626,14828830
g1,178:23216646,14828830
x1,178:25068494,14828830
g1,178:25270514,14828830
x1,178:26347954,14828830
k1,180:31614142,14828830:5266188
g1,180:31614142,14828830
)
(1,186:9664114,15549726:21950028,442260,147420
(1,182:9664114,15549726:0,379288,0
g1,182:9664114,15549726
g1,182:9192734,15549726
g1,182:8865054,15549726
(1,182:8865054,15549726:471380,379288,0
g1,182:8865054,15549726
x1,182:9336434,15549726
)
g1,182:9664114,15549726
)
x1,182:10286917,15549726
g1,183:10488937,15549726
x1,183:10901349,15549726
x1,183:11524243,15549726
x1,183:11844108,15549726
x1,183:12147137,15549726
g1,183:12349157,15549726
x1,183:13325587,15549726
g1,183:13527607,15549726
x1,183:14150410,15549726
g1,183:14352430,15549726
x1,183:17366122,15549726
g1,183:17568142,15549726
x1,183:18722658,15549726
g1,185:18924678,15549726
x1,185:19673790,15549726
x1,185:20384225,15549726
g1,185:20586245,15549726
x1,185:21065997,15549726
g1,185:21268017,15549726
x1,185:21705726,15549726
g1,185:21907746,15549726
x1,185:22605534,15549726
g1,185:22807554,15549726
x1,185:24491052,15549726
g1,185:24693072,15549726
x1,185:25972532,15549726
g1,185:26174552,15549726
x1,185:27251992,15549726
k1,186:31614142,15549726:4362150
g1,186:31614142,15549726
)
(1,192:9664114,16270622:21950028,442260,147420
(1,188:9664114,16270622:303030,379288,0
g1,188:9664114,16270622
g1,188:9192734,16270622
g1,188:8865054,16270622
(1,188:8865054,16270622:774410,379288,0
g1,188:8865054,16270622
x1,188:9639464,16270622
)
g1,188:9967144,16270622
)
x1,188:10589947,16270622
g1,189:10791967,16270622
x1,189:11608417,16270622
x1,189:13224576,16270622
x1,189:13695955,16270622
g1,189:13897975,16270622
x1,189:14520778,16270622
g1,189:14722798,16270622
x1,189:15135210,16270622
x1,189:15758104,16270622
x1,189:16077969,16270622
x1,189:16380998,16270622
g1,189:16583018,16270622
x1,189:17559448,16270622
g1,189:17761468,16270622
x1,189:18384271,16270622
g1,189:18586291,16270622
x1,189:21599983,16270622
g1,189:21802003,16270622
x1,189:26517075,16270622
g1,191:26719095,16270622
x1,191:28032453,16270622
x1,191:29210903,16270622
k1,192:31614142,16270622:2403239
g1,192:31614142,16270622
)
]
(1,194:8865054,45574276:22749088,0,0
h1,194:8865054,45574276:22749088,0,0
)
]
]
!10569
}4
Input:21:D:\Science\2024_ACHEP\samplepaper.aux
!57
Postamble:
Count:2527
!26
Post scriptum:

